AutoFT: Learning an Objective for Robust Fine-Tuning

Foundation models encode rich representations that can be adapted to downstream tasks by fine-tuning. However, fine-tuning a model on one data distribution often degrades performance under distribution shifts. Current approaches to robust fine-tuning use hand-crafted regularization techniques to constrain the fine-tuning process towards the pretrained model. Yet, it is hard to specify how to adapt relevant characteristics of the foundation model during fine-tuning, as this depends on how the pre-training, fine-tuning, and test data distributions relate to each other. We propose AutoFT, a data-driven approach for robust fine-tuning. Given a task, AutoFT searches for a fine-tuning procedure that enhances out-of-distribution (OOD) generalization. Specifically, AutoFT uses bi-level optimization to search for an objective function and hyperparameters that maximize post-adaptation performance on a small OOD validation set. We evaluate AutoFT on nine natural distribution shifts. Our experiments show that AutoFT significantly improves generalization to OOD inputs, outperforming existing robust fine-tuning methods. Notably, AutoFT achieves a new state-of-the-art on the WILDS iWildCam and FMoW benchmarks, outperforming the previous best methods by $6.0\%$ and $1.5\%$, respectively.

==> arxiv/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> arxiv/sections/ablations.tex <==
\textbf{Transferability of the learned objective and hyperparameters.} 
We explore the transferability of hyperparameters learned on one fine-tuning distribution to new distributions.
\ours{} was first applied to CIFAR-10, using $100$ examples from CIFAR-10-C as the OOD validation set.
Using the learned objective and hyperparameters, we then fine-tuned a model on three new distributions -- MNIST, CIFAR-10.1, and CIFAR-10.2, with results shown in \cref{tab:hparam-transfer}.
Additional experimental details are in \cref{sec:app-autoft-details}.
\ours{} outperforms standard fine-tuning in ID and OOD accuracy with both CIFAR-10.1 and CIFAR-10.2, but is less effective on MNIST.
This suggests that the hyperparameters from \ours{} transfer more effectively to distributions similar to the original fine-tuning dataset.


\textbf{Choice of validation set.} 
\begin{table} \centering
\begin{tabular}{lcc}
\toprule
Validation Set & ID Test & OOD Test \\
\midrule
ID Val         & 52.3    & 35.8     \\
OOD Val        & 51.0    & 38.3     \\
OOD Test       & 50.7    & \textbf{39.0} \\
\bottomrule
\end{tabular}
\caption{
\label{tab:val-set-choice}
\textbf{\ours{} performs best with an OOD validation set.} We evaluate \ours{} on iWildCam with various validation sets (ID Val, OOD Val, OOD Test). Non-ID validation sets enhance OOD generalization most.}
\end{table}
How does the choice of validation set affect OOD generalization?
We evaluated \ours{} with different validation sets (ID Val, OOD Val, OOD Test) on the iWildCam benchmark in \cref{tab:val-set-choice}.
Using an ID validation set improves ID performance, while using a non-ID validation set improves OOD performance.
Thus, when optimizing for OOD generalization, using a validation set from a different distribution than the fine-tuning distribution is best.


\textbf{Choice of hyperparameter optimization algorithm.} 
\begin{table} \centering
\begin{tabular}{lcc}
\toprule
                                    & ID Test & OOD Test \\
\midrule
Random                           & 29.8    & 24.5     \\
Quasi Monte Carlo                & 48.2    & 34.7     \\
Bayesian Optimization            & 49.9    & 36.5     \\
Tree-Structured Parzen Estimator & 51.0    & \textbf{38.3}     \\
\bottomrule
\end{tabular}
\caption{\label{tab:hpo_algorithm}
\textbf{\ours{} with different hyperparameter optimization algorithms.} 
We evaluate \ours{} on iWildCam with various hyperparameter optimization algorithms given the same computational budget.
The tree-structured Parzen estimator (TPE) outperforms other methods by a large margin.
}
\end{table}
We conduct an experiment comparing AutoFT with three different hyperparameter optimization methods: random search, quasi Monte Carlo, and Bayesian optimization.
Results in \cref{tab:hpo_algorithm} show that Tree-Structured Parzen Estimator (TPE) is most effective.
% in terms of ID and OOD performance.
% We vary the hyperparameter optimization method used in \ours{}: random search, quasi Monte Carlo, and Bayesian optimization.


\textbf{Effect of validation set size.}
% \begin{table} \centering
% \begin{tabular}{lcc}
% \hline
% No. Examples & ID Test & OOD Test \\
% \hline
% % FLYP          & 52.2    & 35.6     \\
% 200          & 48.9    & 37.2     \\
% 1000         & 51.0    & 38.3     \\
% 5000         & 50.4    & 38.0     \\
% 10000        & 48.9    & 37.8     \\
% \hline
% \end{tabular}
% \caption{
% \label{tab:val-set-size}
% \textbf{Effect of val set size.} 
% Performance of \ours{} on iWildCam with varying validation set sizes. Increasing size beyond $1000$ shows minimal additional benefits.}
% \end{table}
We examine the effect of validation set size on performance in \cref{tab:val-set-size}. 
\ours{} yields improvements in OOD performance compared to the leading fine-tuning baseline (FLYP OOD Test: $35.6\%$) across all validation set sizes.
Given a fixed number of inner steps and hyperparameter evaluations, there's an optimal range for validation set size, beyond which additional benefits are minimal.

\textbf{Learned objective and hyperparameters are dataset-specific.}
\cref{sec:learned-hparams-analysis} reveals differences in learned objectives and hyperparameters between ImageNet and iWildCam tasks. Both tasks prioritize contrastive image-text loss, confidence regularization, and cross entropy losses. Yet, significant variations in L2 norm, weight decay, and learning rate indicate that these learned hyperparameters are task-specific, not universal.

==> arxiv/sections/abstract.tex <==
% Foundation models encode rich representations that can be adapted to downstream tasks by fine-tuning.
% However, fine-tuning a model on one data distribution often degrades performance under distribution shifts.
% Yet, it is hard to specify how to adapt relevant characteristics of the foundation model during fine-tuning, as this depends on how the pre-training, fine-tuning, and evaluation data distributions relate to each other.
% We propose AutoFT, a data-driven approach for guiding foundation model fine-tuning.
% Given a fine-tuning task, AutoFT searches for a fine-tuning procedure that is robust to distribution shifts.
% Specifically, AutoFT uses bi-level optimization to search for an objective function and hyperparameters that maximize final performance on a small out-of-distribution (OOD) validation set.
% We evaluate AutoFT on nine natural distribution shifts, including domain shifts and subpopulation shifts.
% Our experiments show that AutoFT significantly improves generalization to new OOD data, outperforming existing robust fine-tuning methods. 
% Notably, AutoFT achieves a new state-of-the-art on the WILDS-iWildCam and WILDS-FMoW benchmarks, outperforming the previous best methods by 6.0% and 1.5%, respectively.

Foundation models encode rich representations that can be adapted to downstream tasks by fine-tuning.
However, fine-tuning a model on one data distribution often degrades performance under distribution shifts.
Current approaches to robust fine-tuning use hand-crafted regularization techniques to constrain the fine-tuning process towards the pretrained model.
Yet, it is hard to specify how to adapt relevant characteristics of the foundation model during fine-tuning, as this depends on how the pre-training, fine-tuning, and test data distributions relate to each other.
We propose \ours{}, a data-driven approach for robust fine-tuning.
Given a task, \ours{} searches for a fine-tuning procedure that enhances out-of-distribution (OOD) generalization.
Specifically, \ours{} uses bi-level optimization to search for an objective function and hyperparameters that maximize post-adaptation performance on a small OOD validation set.
% \ours{} searches for a fine-tuning procedure that maximizes performance on a small out-of-distribution (OOD) validation set.
% Specifically, \ours{} searches a highly expressive hyperparameter space that includes weights for several different losses, in addition to learning rate and weight decay.
We evaluate \ours{} on nine natural distribution shifts.
Our experiments show that \ours{} significantly improves generalization to new OOD data, outperforming existing robust fine-tuning methods. 
Notably, \ours{} achieves a new state-of-the-art on the WILDS iWildCam and FMoW benchmarks, outperforming the previous best methods by $6.0\%$ and $1.5\%$, respectively.

% Yet, it is hard to precisely specify what characteristics of the foundation model to retain during fine-tuning, as this depends on how the pre-training, fine-tuning, and evaluation data distributions relate to each other.

==> arxiv/sections/background.tex <==
We first formalize hyperparameter optimization as a means for searching the space of fine-tuning procedures in \cref{sec:method}.
Hyperparameters are predefined properties of the learning algorithm which are not learned during training, such as network architecture, learning rate, and regularization strength.
A good choice of hyperparameters can significantly improve model performance, yet optimal hyperparameters vary, depending on the data distribution and evaluation metrics.
% Hyperparameters significantly impact the performance of the final model; thus, choosing the right hyperparameters is important. 
% It is difficult to know the optimal hyperparameters a priori, as they are influenced by many properties of the problem setting, including the data distribution and desired evaluation metric.
% It is difficult to know the optimal hyperparameters a priori, as they depend on many properties of the problem setting, including the data distribution and desired evaluation metric.

Formally, we denote the learning algorithm as $\LA$ and its hyperparameters as $\phi \in \Phi$, where $\Phi$ is the hyperparameter space.
We denote the training and validation datasets as $\Dtr$ and $\Dval$, respectively.
These datasets are disjoint and typically drawn from the same distribution.
The learning algorithm $\LA$ produces a model by training on $\Dtr$ with hyperparameters $\phi$.
We denote the resulting model as $\LA(\phi, \Dtr)$.
% , to explicitly represent the dependence on both hyperparameters $\phi$ and training data $\Dtr$.
% The goal of hyperparameter optimization is to find hyperparameters that maximize some performance metric $\mathrm{Perf}(f, \Dval)$ which depends on the model $f$ and the validation dataset $\Dval$.
Hyperparameter optimization finds hyperparameters that maximize some performance metric $\mathrm{Perf}(f, \Dval)$ which depends on the model $f$ and the validation dataset $\Dval$.
Examples of performance metrics include top-1 accuracy, macro F1 score, and worst-region accuracy.
We formalize hyperparameter optimization as
% \begin{equation}
%     \label{eq:hyperopt}
% \phi^* = \argmax_{\phi \in \Phi} \mathbb{E} [\mathrm{Perf}(\LA(\phi, \Dtr), \Dval)].
% \end{equation}
\begin{equation}
    \label{eq:hyperopt}
    \phi^* = \argmax_{\phi \in \Phi} \mathbb{E} \big[ \overbrace{\mathrm{Perf}(\underbrace{\LA(\phi, \Dtr)}_{\text{Learned Parameters}}, \Dval)}^{\text{Validation Set Performance}} \big].
\end{equation}
Here, the expectation is taken over any randomness in the learning algorithm $\LA$, such as input data shuffling or random initialization.
The optimized hyperparameters $\phi^*$ are subsequently used to train the model.

Hyperparameter optimization methods typically start with randomly initialized model parameters and use a validation set $\Dval$, drawn from the same distribution as the training data, to adjust hyperparameters.
The problem of robust fine-tuning, however, begins with pre-trained model parameters and aims to achieve high performance on test data that diverges from the fine-tuning distribution.
In the next section, we describe how we leverage hyperparameter optimization to learn a robust adaptation procedure.
% In the next section, we describe how we modify the standard hyperparameter optimization loop to robustly fine-tune foundation models.
% This involves using non-IID validation datasets $\Dval$ to anticipate distribution shift at test time.

%%CF.11.15: I think it would be good to explicitly point out, maybe here at the end, that prior hyperparameter optimization approaches typically use a validation set D_val that is sampled iid from the training distribution, alongside random initial parameters. + how in the next section, we will describe how we will extend hyperparameter optimization to the setting of fine-tuning pre-trained foundation models, and consider non-IID D_val datasets.

==> arxiv/sections/experimental_setup.tex <==
\textbf{Evaluation.} We fine-tune pre-trained CLIP models from the \texttt{open-clip} repository~\citep{radford2021learning,ilharco_gabriel_2021_5143773}. 
We use the CLIP \texttt{ViT-B/16} model from OpenAI as our default model, unless specified otherwise.
% Evaluation on CIFAR-10 use the CLIP \texttt{ViT-L/14} model from OpenAI, in line with \citet{wortsman2022robust}.
Our SoTA results on WILDS-iWildCam and WILDS-FMoW use the CLIP \texttt{ViT-L/14-336px} model.
We use text templates used in prior work~\citep{radford2021learning,wortsman2022robust} to generate zero-shot classification weights.

Following prior works on robust fine-tuning, we evaluate \ours{} on nine \textit{natural distribution shifts}, few-shot learning, and transfer learning settings \cite{taori2020measuring, radford2021learning, wortsman2022robust, kumar2022fine, goyal2022finetune}.
% \citet{} as shifts arising from real-world variations, such as changes in lighting, geography, and image styles. 
% This approach, in line with prior works on robust fine-tuning \citep{radford2021learning, wortsman2022robust, kumar2022fine, goyal2022finetune}, emphasizes shifts that are representative of real-world scenarios.
These include five ImageNet distribution shifts (IN-V2, IN-R, IN-Sketch, ObjectNet, and IN-A) \citep{recht2019imagenet, hendrycks2021many, wang2019learning, barbu2019objectnet, hendrycks2021natural}, WILDS-iWildCam \citep{koh2021wilds,beery2021iwildcam}, WILDS-FMoW \citep{koh2021wilds,christie2018functional}, CIFAR-10.1 \citep{recht2018cifar10.1, torralba2008tinyimages}, and CIFAR-10.2 \citep{lu2020harder}. 
We use up to $1000$ examples from ImageNet-C, OOD validation splits of WILDS-FMoW and WILDS-iWildCam, and CIFAR-10-C as the OOD validation sets.
We also evaluate on few-shot classification (\cref{tab:fewshot-binary-classification} and \cref{fig:imagenet-fewshot-effective-robustness-plots}) and transfer learning (\cref{tab:transfer_learning}).
% The WILDS-iWildCam dataset \citep{beery2021iwildcam, koh2021wilds, sagawa2022extending} presents distribution shifts arising from variations in camera trap locations, lighting conditions, and animal behaviors across various geographic regions. 
% The WILDS-FMoW dataset \citep{christie2018functional, koh2021wilds, sagawa2022extending} presents distribution shifts arising from changes in time, geographic locations, and land use.
% The CIFAR-10.1 and CIFAR-10.2 shifts involve subtle changes in image characteristics and composition. 

% \textbf{Foundation models and CLIP.} 

\begin{table}[b]
\vspace{-3mm}
\centering
\begin{tabular}{lccc}
\toprule
\textbf{Dataset} & \textbf{Steps} & \textbf{Trials} & \textbf{$N_\textrm{val}$} \\
\midrule
iWildCam & 10 & 500 & 1000 \\
FMoW & 10 & 500 & 1000 \\
CIFAR-10 & 10 & 100 & 100 \\
Flowers & 50 & 500 & 500 \\
Cars & 50 & 500 & 1000 \\
ImageNet & 100 & 500 & 1000  \\
\bottomrule
\end{tabular}
\caption{\label{tab:hyperhyper}
\ours{} training settings for each dataset.
}
\end{table}

\textbf{Effective robustness and weight ensembling curves.} 
We primarily evaluate robustness to distribution shifts using average OOD performance.
We also compare methods with weight ensembling of the zero-shot and fine-tuned models \citep{wortsman2022robust}, which enhances ID and OOD performance in a way orthogonal to fine-tuning.
We interpolate model weights with ten mixing coefficients, \( \alpha \), and report results using the coefficient that maximizes ID validation accuracy.
Finally, we plot ID and OOD performance across these different interpolation coefficients in \cref{fig:effective-robustness-plots} to visualize \textit{effective robustness} -- gains in accuracy beyond the zero-shot model, which corresponds to \textit{vertical distance} between curves.

\textbf{Baselines.} 
We compare \ours{} against several methods for adapting pretrained models. 
We include two standard transfer learning methods that minimize cross-entropy loss: linear probing (LP) and full fine-tuning (FT).
We also compare with recent works in robust fine-tuning: 
L2-SP~\citep{li2018massively}, which fine-tunes with an L2 regularization term towards pretrained weights; 
LP-FT~\citep{kumar2022fine}, which performs linear probing followed by full fine-tuning; 
Freeze-Embed~\citep{kumar2022sgdfinetuning}, which freezes the embedding layer during fine-tuning;
and FLYP~\citep{goyal2022finetune}, which fine-tunes with the CLIP pretraining loss -- a contrastive loss between image embeddings and class-descriptive prompt embeddings.
As we are interested in OOD performance, we also compare against OOD generalization methods, including Group DRO~\citep{sagawa2019distributionally}, ABSGD~\citep{qi2020attentional}, LISA~\citep{yao2022improving}, DFR~\citep{kirichenko2022last}, and Copy-Paste~\citep{gao2023out}.
We additionally evaluate all methods with weight ensembling (WiSE-FT)~\citep{wortsman2022robust}, which is shown to improve OOD performance in an orthogonal way to other robust fine-tuning methods.

\textbf{Bi-level optimization details.} 
We summarize the number of inner-loop gradient steps, outer-loop fine-tuning trials, and validation set size for each dataset in \cref{tab:hyperhyper}.
All of these values were selected based on performance on an ID validation set.
% We report the number of inner-loop gradient steps, \texttt{Optuna} trials we use in hyperparameter optimization as follows.
We provide additional details on our training protocol in~\cref{sec:appendix-hyperparams}.


==> arxiv/sections/experiments_old.tex <==
\subsection{Experimental Setup}
\textbf{Datasets.} 
We evaluate \ours{} on a wide array of datasets with a distribution shift between training and test.
The datasets we consider include both synthetic and real-world distribution shifts.
Below, we summarize the datasets we use for evaluation, including the fine-tuning dataset (ID), the validation dataset for hyperparameter optimization, and the test OOD datasets.

\begin{itemize}
    \item \textbf{CIFAR-10} \citep{krizhevsky2009learning} contains 60,000 images across 10 classes.
    We use CIFAR-10 for fine-tuning, 100 examples from CIFAR-10-C for validation, and the CIFAR-10.1~\citep{recht2018cifar10.1,torralba2008tinyimages} and CIFAR-10.2~\citep{lu2020harder} as OOD test sets.

    \item \textbf{ImageNet} ~\citep{deng2009imagenet} contains over a million images in 1000 categories. 
    We use ImageNet as our ID distribution, 15000 examples from ImageNet-C for validation, and five ImageNet variations for the OOD datasets following prior works~\citep{clip,wortsman2022robust,kumar2022fine,goyal2022finetune}: ImageNet-V2~\citep{recht2019imagenet}, ImageNet-R~\citep{hendrycks2021many}, ImageNet-A~\citep{hendrycks2021natural}, ImageNet-Sketch~\citep{wang2019learning}, and ObjectNet \citep{barbu2019objectnet}.
    
    \item \textbf{WILDS-iWildCam} \citep{beery2021iwildcam, koh2021wilds, sagawa2022extending} is an animal image classification dataset with 182 classes. 
    Differences in camera specifications and attributes such as background and lighting distinguish ID and OOD.
    We use the ID train set from \citet{koh2021wilds} as the fine-tuning dataset, the OOD validation set for hyperparameter optimization, and the OOD test set for evaluation.

    \item \textbf{WILDS-FMoW} \citep{christie2018functional, koh2021wilds, sagawa2022extending} contains remote sensing imagery from satellites. 
    Each image is to be classified into one among 62 categories, including labels like ``impoverished settlement'' and ``hospital''.
    The ID and OOD datasets differ in time of acquisition and geographic location.
    We use the ID train set for fine-tuning, the OOD validation set for hyperparameter optimization, and the OOD test set for evaluation.

In all of the transfer learning datasets described below, we use a portion of the validation set for hyperparameter optimization.
    \item \textbf{Caltech101} \citep{fei2004learning} contains images of objects from 101 different categories, including ``dragonfly'', ``grand piano'', and ``saxophone.''

    \item \textbf{StanfordCars} \citep{krause20133d} features a collection of car images categorized by model, make, and year, where the task is to classify them into one of 196 types, such as ``Ford Mustang Convertible 1967'' or ``Toyota Prius Hatchback 2009.''

    \item \textbf{Flowers102} \citep{veeling2018rotation} consists of flower images from the UK, with the objective of classifying each image into one of 102 species, such as ``oxeye daisy'' or ``hibiscus.''

    \item \textbf{PatchCamelyon} \citep{veeling2018rotation} provides digital pathology images for binary classification, with the goal of identifying metastatic tumor tissues.

    \item \textbf{Rendered SST2} \citep{radford2021learning} is a dataset for optical character recognition, where the task is to classify text sentiment as ``positive'' or ``negative.''
    
\end{itemize}

\vspace{2mm} \noindent 
\textbf{Baselines.} 
We compare \ours{} against several methods for adapting pretrained models. 
We include two standard transfer learning methods that minimize cross-entropy loss: linear probing (LP) and full fine-tuning (FT).
We also compare with recent works in robust fine-tuning: L2-SP~\citep{li2018massively}, which fine-tunes with an L2 regularization term towards pretrained weights; LP-FT~\citep{kumar2022fine}, which performs linear probing followed by full fine-tuning; and FLYP~\citep{goyal2022finetune}, which fine-tunes with a contrastive loss.
We additionally evaluate all methods with weight ensembling~\citep{wortsman2022robust}, which is shown to improve OOD performance in an orthogonal way to other robust fine-tuning methods.

\vspace{2mm} \noindent 
\textbf{Models.} 
We fine-tune pre-trained CLIP~\citep{radford2021learning} models, including those provided in the \texttt{open-clip} repository~\citep{ilharco_gabriel_2021_5143773}. 
We use the CLIP ViT-B/16 model from OpenAI as our default model, unless specified otherwise. 
The CIFAR-10 experiments use the CLIP ViT-L/14 model from OpenAI.

\vspace{2mm} \noindent 
\textbf{Training.} 
We closely follow the training procedure described in~\citep{goyal2022finetune}.
All methods fine-tune models with an AdamW optimizer and a cosine learning rate scheduler. 
We use a batch size of 512 for ImageNet and 256 for all other datasets. 
For all baselines, we use learning rate and weight decays tuned through grid search and implement early stopping based on in-distribution (ID) validation accuracy. 
We note that all methods, including \ours{}, do not observe any of the test OOD datasets at training.
We report average metrics over 5 runs with 95\% confidence intervals. 
We use text templates used in prior work~\citep{radford2021learning,wortsman2022robust} to generate zero-shot final layer weights for all datasets.
A comprehensive breakdown of hyperparameter sweeps can be accessed in Appendix B.

\vspace{2mm} \noindent 
\textbf{\ours{}-specific settings.} 
% \ours{} uses a validation dataset different from both the reference (ID) dataset and the test OOD datasets for hyperparameter optimization.
As described in~\cref{sec:method}, \ours{} learns weights for nine different losses on a log-uniform range $[\text{1e-4},\text{1e2}]$, learning rate in the log-uniform range $[\text{1e-7},\text{1e-3}]$, and weight decay in the log-uniform range $[0.0, 1.0]$.
The layerwise variant of \ours{} learns per-layer learning rates and weight decay regularization terms, each sampled from the same respective range.
\todo{Add optuna hyperparames: inner loop steps, outer loop steps}

\subsection{Evaluation Under Distribution Shifts}

To evaluate the effectiveness of \ours{} in adapting pretrained models to new tasks, we compare against baselines on several large-scale, real-world distribution shift benchmarks, including ImageNet, WILDS-iWildCam, and WILDS-FMoW.
We report weight ensembling results with the mixture coefficient that attains the highest ID validation accuracy.
We report macro F1 score for WILDS-iWildCam and worst-region accuracy for WILDS-FMoW, following \citet{koh2021wilds}.

We report the ID and OOD test metrics of all methods in \cref{tab:big_distribution_shift_table}.
We find that \ours{} consistently outperforms all baselines on unseen OOD test distributions.
Additionally, these gains in OOD performance are preserved when ensembling the zeroshot and fine-tuned models, as proposed by \citet{wortsman2022robust}.

\textcolor{blue}{\ours{} attains a new state of the art on WILDS-iWildCam by $XXX\%$ in OOD Macro F1 score, using a ViT-L/14@336px backbone.}
With a ViT-B/16 model, \ours{} improves OOD performance by XXX\% over full fine-tuning (FT) and XXX\% over the current state-of-the-art, FLYP. 

Our experiments demonstrate that \ours{} consistently improves effective robustness on ImageNet, WILDS-iWildCam, and WILDS-FMoW compared to baseline methods.
\ours{} achieves superior out-of-distribution (OOD) accuracy compared to baseline methods for any given in-distribution (ID) accuracy on ImageNet.

\textbf{Weight ensembling curves.} We use the \textit{effective robustness} framework by \citet{taori2020measuring} to evaluate model robustness based on accuracy exceeding a baseline trained only on the reference distribution.

Linearly interpolating the weights of a fine-tuned model and a pretrained model (WiSE-FT) has been shown to improve both ID and OOD performance \citep{wortsman2022model}.
Hence, we include weight ensembling as an additional point of comparison, and interpolate the weights of models fine-tuned by each method with 10 mixing coefficients $\alpha$.
We use scatter plots to display effective robustness and plot the reference distribution accuracy (ID) against the shift accuracy (OOD) at various mixing coefficients.


\textbf{ImageNet distribution shifts.}

\textbf{WILDS distribution shifts.} 
We evaluate \ours{} on WILDS-iWildCam and CIFAR-10 distribution shifts in ~\cref{tab:iWildCam_no_ensembling_data_table} and ~\cref{tab:cifar10}, respectively.
\ours{} outperforms several representative methods for robust fine-tuning on unseen OOD data.

\input{tables/big_table.tex}

\textbf{CIFAR distribution shifts.}  We evaluate \ours{} on a CIFAR-10 derived distribution shift task and report results in ~\cref{tab:cifar10}.
We find that \ours{} outperforms several representative methods for robust fine-tuning on unseen synthetic OOD data.

\begin{table*}
\centering
\begin{tabular}{ccc}
\toprule
Method & CIFAR-10.1 & CIFAR-10.2 \\
\midrule
Zero-shot & 92.5 & 88.8 \\
Fine-tuning & 95.9 & 91.3 \\
\oursbf & \textbf{97.5} & \textbf{93.5} \\
\midrule
% WiSE-FT ($\alpha=0.5$) & 97.6 & 93.4 \\
WiSE-FT (best $\alpha$) & 98.0 & 94.4 \\
\oursbf w/ weight ensembling (best $\alpha$) & \textbf{98.3} & \textbf{95.0} \\
\bottomrule
\end{tabular}
\caption{CIFAR-10 results.}
\end{table*}


\begin{table*}[t] \centering
\begin{minipage}{.56\textwidth} \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{ccc}
    \toprule
    Method & CIFAR-10.1 & CIFAR-10.2 \\
    \midrule
    Zero-shot & 92.5 & 88.8 \\
    Fine-tuning & 95.9 & 91.3 \\
    \oursbf{} & \textbf{97.5} & \textbf{93.5} \\
    \midrule
    % WiSE-FT ($\alpha=0.5$) & 97.6 & 93.4 \\
    WiSE-FT (best $\alpha$) & 98.0 & 94.4 \\
    \oursbf{} w/ weight ensembling (best $\alpha$) & \textbf{98.3} & \textbf{95.0} \\
    \bottomrule
    \end{tabular}
    }
    \caption{
    \ours{} outperforms fine-tuning by $2.2\%$ on CIFAR-10.2 and by $1.4\%$ on CIFAR-10.1, using only 100 samples from CIFAR-10-C.
    \ours{} additionally outperforms WiSE-FT with weight ensembling.}
    \label{tab:cifar10}
\end{minipage}%
\hfill
\begin{minipage}{.42\textwidth} \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{cccc}
    \toprule
    Validation Dataset & CIFAR-10.1 & CIFAR-10.2 \\
    \midrule
    CIFAR-10-C & 97.4 (0.2) & 93.5 (0.2) \\
    CIFAR-10 & 96.9 (0.2) & 93.2 (0.1) \\
    CIFAR-10.1 & 96.8 (0.3) & 92.8 (0.2) \\
    CIFAR-10.2 & 96.7 (0.5) & 93.8 (0.0) \\
    \bottomrule
    \end{tabular}
    }
    \caption{
    ID and OOD performance of \ours{} using various validation sets for hyperparameter optimization.
    \ours{} uses just 100 samples from each of CIFAR-10-C, CIFAR-10, CIFAR-10.1, and CIFAR-10.2.}
    \label{tab:varying_validation_sets}
    \end{minipage}
\end{table*}


\subsection{Few-Shot Classification}

Few-shot classification is a critical benchmark for assessing the practicality of zeroshot models in many real-world applications, where limited labeled fine-tuning data is available.
\ours{} effectively generalizes given small quantities of labeled data, making it a promising approach for fine-tuning in low-data regimes.
\ours{} improves upon state-of-the-art fine-tuning methods in few-shot learning, resulting in gains of up to $5.1\%$ and $4.0\%$ on the SST2 and PatchCamelyon benchmarks, respectively.

\subsubsection{Binary Few-Shot Classification}

In few-shot binary classification, the small number of training examples present a challenging task for adaptation.
Our evaluation encompasses two datasets: PatchCamelyon and Rendered-SST2, replicating the experimental setup of \citet{radford2021learning}.
\ours{} significantly improves upon existing fine-tuning approaches in 4, 16, and 32 shot classification, as shown in \cref{tab:fewshot-binary-classification}. 
For example, \ours{} outperforms FLYP by $3.7\%$ and traditional full fine-tuning by $3.9\%$ in a difficult 4-shot classification task on SST2.

\input{tables/fewshot_binary.tex}

% \subsubsection{ImageNet Few-Shot Classification}

\subsection{Transfer Learning}


\input{tables/transfer_learning.tex}


Does \ours{} improve performance even when the test distribution is the same as the fine-tuning distribution?
We consider the more general transfer learning setup, where a model trained on one dataset is applied to a different, but related, dataset, with the aim of achieving high in-distribution accuracy.
\ours{} improves performance on XX out of XX transfer learning datasets, compared to several state-of-the-art fine-tuning methods.

In \cref{tab:transfer_learning}, we benchmark \ours{} against other models on six transfer learning datasets: PatchCamelyon, CalTech101, StanfordCars, Flowers102, ImageNet, and iWildCam. 
\ours{} shows superior generalization across all six datasets. For instance, \ours{} improves performance by $XX.XX\%$ than XXX baseline on XXX dataset and $XX.XX\%$ on XXX.


\subsection{Transferability of Hyperparameters} 

\subsection{Varying the Hyperparameter Optimization Dataset} 
We evaluate the performance of \ours{} using different validation datasets in \cref{tab:varying_validation_sets}.
While our main results optimize hyperparameters using a held-out validation set from a distribution that is different from the ID and test OOD distributions, here we use both a held-out ID validation set and a held-out OOD validation set.
We find that \ours{} exhibits strong test OOD performance with several different hyperparameter optimization datasets.
However, the best test OOD performance is attained with a validation set that is from a different distribution than the ID dataset.

% \begin{table}[]
% \centering
% \begin{tabular}{cccc}
% \toprule
% Validation Dataset & CIFAR-10.1 & CIFAR-10.2 \\
% \midrule
% CIFAR-10-C & 97.4 (0.2) & 93.5 (0.2) \\
% CIFAR-10 & 96.9 (0.2) & 93.2 (0.1) \\
% CIFAR-10.1 & 96.8 (0.3) & 92.8 (0.2) \\
% CIFAR-10.2 & 96.7 (0.5) & 93.8 (0.0) \\
% \bottomrule
% \end{tabular}
% \caption{
% ID and OOD performance of \ours{} using various validation sets for hyperparameter optimization.
% \ours{} uses just 100 samples from each of CIFAR-10-C, CIFAR-10, CIFAR-10.1, and CIFAR-10.2.}
% \label{tab:varying_validation_sets}
% \end{table}


% \subsection{Transferring Learned Hyperparameters Across Datasets}
% 1. Learned on CIFAR-10 -> CIFAR-10-C, finetune on CINIC, evaluate on CIFAR-10.1,10.2?

% 2. Learned on CIFAR-10 -> CIFAR-10-C, finetune on MNIST, evaluate on RMNIST,CMNIST,EMNIST,etc.?

% \input{tables/iWildCam}
% iWildCam state-of-the-art~\cref{tab:sota_iwild}

==> arxiv/sections/method.tex <==
% To adapt hyperparameter optimization for robust fine-tuning, we utilize three core insights.
% First, we consider a larger hyperparameter space. 
% We extend the definition of ``hyperparameter" to include (per-layer) weight coefficients for nine varied loss functions and regularizers, learning rates, and weight decays.
% Second, we perform hyperparameter optimization on an OOD validation set rather than an ID validation set. 
% Third, performance on one OOD distribution serves as a good proxy for performance on other unseen OOD distributions.
% This eliminates the need to optimize hyperparameters over an exhaustive list of OOD datasets, reducing the complexity and computational cost of hyperparameter optimization.

% summary and motivation
In this section, we present \ours{}, a data-driven approach for robust fine-tuning.
Given a foundation model and task-specific data, \ours{} uses bi-level optimization to learn a fine-tuning objective and optimal hyperparameters.
There are two key contributions in \ours{}.
First, learning the fine-tuning objective enables a more precise adaptation to task-specific data.
% strike a better balance between the general-purpose knowledge encoded in the pre-trained model and the task-specific knowledge in the training data.
Second, \ours{} optimizes the objective and hyperparameters for performance under a proxy distribution shift, which enhances OOD generalization.

\subsection{Problem Setting: Robust Fine-Tuning}

% Data assumptions
\textbf{Data assumptions.} We assume access to two datasets:
(1) a large fine-tuning dataset $\Dtr$ from the training distribution $\Ptr$, and 
(2) a small held-out OOD validation set $\Dval$ from a different distribution $\Pval$.
The validation set $\Dval$ is much smaller than $\Dtr$, containing up to $1000$ examples, and is only used for outer-level optimization, not for fine-tuning.
We then fine-tune on $\Dtr$ with the found hyperparameters and test the fine-tuned model on several OOD distributions $\Pood^1, \Pood^2, \dots$.
Note that these test distributions are distinct from both $\Ptr$ and $\Pval$, and are never shown to the model before final evaluation.
Following prior works on robust fine-tuning, all distributions are assumed to be related to the same task.
We consider domain and subpopulation shifts arising from differences in data collection. 
For instance, in animal recognition from camera trap images, each distribution may represent different locations \citep{beery2021iwildcam,koh2021wilds}.
% Our approach requires minimal data (at most $1000$ examples) from a held-out distribution.
Such data is often readily available, as shown in the WILDS and DomainBed benchmarks \citep{koh2021wilds,gulrajani2020search}, and can be constructed by partitioning by time or geographical location.

\textbf{Notation and concrete setup.} 
Let $f$ denote a pre-trained foundation model with parameters $\theta$, which we adapt by fine-tuning on $\Dtr$.
We denote the fine-tuning algorithm as $\LA(\phi, \Dtr)$, where $\phi$ specifies both the fine-tuning objective and other hyperparameters such as learning rate.
% Let $\phi \in \Phi$ represent the hyperparameters for fine-tuning, and let $\LA(\phi, \Dtr)$ denote the fine-tuning algorithm which produces adapted model parameters.
% In this work, the fine-tuning algorithm $\LA$ is stochastic gradient descent.
In our experiments, the performance metric $\mathrm{Perf}$ follows the standards in each evaluation setting and is either top-1 accuracy, worst-region accuracy, or macro F1.
% Further details about our experimental setup are in in~\cref{sec:experiments}.

%%CF.11.15: I can't remember if the intro belabored this point already, but I think it would be nice to discuss why we might expect things to work when you have just one OOD D_val and want to generalize to multiple novel OOD distributions. Or maybe we don't expect it persay, but we could forward reference the key finding in the experiments. Relatedly, I think it would be good to briefly discuss here the intuition about how we will need to be careful about how many hyperparameters we optimize because we could overfit to D_val. x

\input{tables/alg.tex}

% \subsection{Bi-level Optimization}
\subsection{Learning a Fine-Tuning Objective via Bi-Level Optimization}

% \todo{rename as bi-level optimization, tone down we learn XXX hparams and rephrase as we learn the loss function as XXX}

% \todo{move hparam details to experimental details in appendix}

%%CF.11.15: I think it would be nice to use paragraph headers to separate out the hyperparameter optimization description, the description on the choice of hyperparameters, and the choice of optimizer. There is a lot of different and interesting design choices when it comes to the choice of hyperparameters in particular, and it would be good to convey that this space of design choices is fairly open, beyond even what we consider in the paper, and that exploring other hyperparameter choices would make for interesting future work. Putting in paragraph headers and also discussing this verbally would make it more explicitly clear that these design choices are separate.

\textbf{Formulation.}
We frame the problem of learning a fine-tuning objective as a bi-level optimization problem with the form~\cref{eq:hyperopt}, which we can solve using existing black-box hyperparameter optimizers.
% Given a hyperparameter space $\Phi$ for a fine-tuning algorithm $\LA$, we solve the optimization problem in~\cref{eq:hyperopt} to find hyperparameters $\phi^*$ such that the fine-tuned model $f^{\prime} = \LA(\phi^*, \Dtr)$ performs well on the OOD validation set $\Dval$.
Practically, solving this bi-level optimization problem involves fine-tuning the same foundation model multiple times, each time with different ``hyperparameters'' $\phi^1, \phi^2, \ldots$ to obtain different final fine-tuned models $f^1=\LA(\phi^1, \Dtr), f^2=\cdots$. 
We then evaluate the quality of each $\phi^i$ through the performance of $f^i$ on the OOD validation set; by aggregating the information from these different fine-tuning runs, we can fine good hyperparameters $\phi^*$.
% The hyperparameter optimization algorithm aggregates the information from these different fine-tuning runs and estimates the best hyperparameters $\phi^*$.
%%CF.11.15: Please also describe what happens at test time with our method. x
At test time, we fine-tune the initial foundation model with $\phi^*$ and evaluate its performance on novel OOD distributions to assess its generalization capabilities.
%%CF.11.15: I worry that this is too short for the reader to full grok, especially given that the idea isn't _that_ intuitive. After making some revisions, it would be good to some more unfamiliar eyes on the text to see if people understand the algorithm after reading sections 3 and 4. x
We summarize this procedure in Algorithm~\ref{alg:hyperopt}.

\textbf{Parameterization of the fine-tuning objective.} 
The main novelty of \ours{} is that we parameterize the fine-tuning objective, which allows outer-loop optimization to search over an expressive space of fine-tuning algorithms.
% We consider a larger hyperparameter space $\Phi$ than what is typically considered.
This extra expressivity is important: for robust fine-tuning, the algorithm must selectively \textit{ignore} some aspects of the training distribution in order to better generalize to novel OOD distributions.
% To enable this more nuanced behavior, we increase the expressivity of the hyperparameter optimization process by expanding the hyperparameter space $\Phi$.
Specifically, we allow $\Phi$ to express the fine-tuning objective by learning weights for a pre-defined set of loss functions and regularizers.
Note that the cross-entropy and hinge losses similarly guide the model's predictions towards the correct label, but with a different amount of penalty for severely incorrect samples.
As another example, the contrastive loss on image-text pairs~\citep{radford2021learning,goyal2022finetune} also guides the model's predictions towards the correct label, but in a way that incorporates language embeddings, which is entirely different from how the cross-entropy and hinge losses operate.
% Similarly, different losses for reducing overconfidence or constraining model parameters towards their initial values have different effects on the model's adaptation process.

Therefore, we consider weight coefficients for nine different loss functions and regularizers: cross-entropy loss, hinge loss, image-text contrastive loss, entropy, confidence minimization, L1 norm, L2 norm, L1 and L2 distance to pretrained model parameters.
We select these losses to address various aspects of model learning and generalization, such as classification accuracy, decision confidence, and prevention of overfitting, ensuring a nuanced and effective model adaptation.
We denote these loss weight coefficients as $W = \{w_1, w_2, \dots, w_9\}$.
Denoting the $i$-th loss function or regularizer as $\mathcal{L}_i$, the total loss $\mathcal{L}$ is the weighted sum $\mathcal{L} = \sum_{i=1}^{9}w_i \mathcal{L}_i$.
To enable finer control over the speed and stability of adaptation during fine-tuning, we additionally learn hyperparameters for the fine-tuning optimizer: learning rate $\eta$, weight decay $\delta$, and random seed $\sigma$.
% For an even larger hyperparameter space, we optionally consider per-layer hyperparameters for the learning rate, weight decay, and parameter norm weights; we call this variant ``per-layer'' in our experiments in \cref{sec:appendix}.
Our complete set of hyperparameters for outer-loop optimization is thus $\phi=(W, \eta, \delta, \sigma)$.

\textbf{Bi-level optimization algorithm.} 
We need a black-box optimizer that can effectively search through the high-dimensional hyperparameter space $\Phi$.
% Finding effective hyperparameters for robust fine-tuning requires an optimizer that can efficiently search our large, high-dimensional hyperparameter space $\Phi$.
We use the Tree-structured Parzen Estimator~\citep[TPE]{NIPS2011_86e8f7ab} for this purpose, as its design allows for efficient processing in high-dimensional spaces and yields effective results at the order of hundreds of evaluations.
TPE creates a probabilistic model from previous hyperparameter evaluations, and differentiates between better and worse hyperparameter configurations by comparing their likelihood under two separate models.
We use the TPE implementation from the \texttt{optuna} library~\citep{akiba2019optuna}. 
Experiments in~\cref{tab:hpo_algorithm} demonstrate that in the context of learning a fine-tuning objective, TPE outperforms other bi-level optimizers such as random search, quasi Monte Carlo, and Bayesian optimization.

% with no further modifications.
%%CF.11.15: Can you briefly motivate this choice before describing it? Why do you use this optimizer? x
As the prior distribution for TPE, we use an appropriately scaled distribution for each hyperparameter, operating in log-space for the weight coefficients and learning rate since the optimal values can vary over several orders of magnitude:
% \begin{align*}
%   w_i \sim \text{LogUniform}&(w_{\text{min}}, w_{\text{max}}),  \\
%   \eta \sim \text{LogUniform}&(\eta_{\text{min}}, \, \eta_{\text{max}}), \
%   \delta \sim \text{Uniform}(0.0, 1.0), \\
%   \rho &\sim [0, 100].
% \end{align*}
\begin{align*}
  w_i \sim \text{LogUniform}(w_{\text{min}}, w_{\text{max}}), \quad &\rho \sim [0, 100]  \\
  \eta \sim \text{LogUniform}(\eta_{\text{min}}, \eta_{\text{max}}), \quad &\delta \sim \text{Uniform}(0.0, 1.0). 
\end{align*}
We find that in practice, $(w_{\text{min}}, w_{\text{max}}) = (10^{-4},10)$ is an effective range for all $w_i$.
Given a model's conventional learning rate $\eta^*$, we set $(\eta_{\text{min}}, \eta_{\text{max}}) = (10^{-2} \eta^*, 10^2 \eta^*)$.

\textbf{Intuition for OOD evaluation.} % To learn a robust fine-tuning objective,  one small OOD validation set $\Dval$ can guide the model to generalize better to various new OOD distributions.
% Performance on this set can serve as an effective proxy for performance on novel OOD distributions.
Optimizing the objective with respect to performance on a small out-of-distribution (OOD) validation set $\Dval$ can guide the model to learn more generalizable parameters during fine-tuning.
% Performance under this distribution shift can serve as an effective proxy for performance under other distribution shifts.
We conduct a didactic toy experiment in~\cref{sec:didactic-experiment}, which illustrates our key intuition: a small validation set reveals \textit{how} the data distribution changes under natural shifts, informing how best to adapt a given foundation model.
% \todo{in one sentence explain the takeaways from the toy experiment}
Our experiments in \cref{sec:results} confirm that \ours{} consistently improves generalization to novel OOD distributions, outperforming state-of-the-art methods.

\textbf{Computational cost.} 
The bi-level optimization of \ours{} introduces minimal computational overhead, requiring at most $5\%$ additional compute compared to one standard fine-tuning run on most benchmarks.
Each evaluation of the objective and hyperparameters requires a small number of inner loop gradient steps on the fine-tuning dataset.
% For example, on the iWildCam dataset, \ours{} uses only 500 hyperparameter evaluations, each requiring only 10 gradient steps on the fine-tuning data. 
% With 1.3 million training examples and a batch size of 256, \ours{} requires only 5000 additional gradient steps, compared to approximately 100,000 gradient steps for final fine-tuning.
\ours{} is therefore computationally inexpensive, and highly practical for even large fine-tuning problem settings.
Hyper-hyperparameters are detailed in \cref{sec:appendix-hyperparams}.


==> arxiv/sections/related.tex <==

\section{Related Work}
\textbf{Transfer learning.}
While early research demonstrated that using features learned from pre-training on large datasets are effective for new tasks, transfer learning has evolved to optimize performance in settings with limited data ~\citep{oquab2014learning,yosinski2014transferable,sharif2014cnn}. 
Common transfer learning techniques include fine-tuning with regularization~\citep{zhang2020side,xuhong2018explicit,lee2019mixout,jiang2019smart,Li2020Rethinking,aghajanyan2020better,gouk2021distancebased,shen2021partial, KARANI2021101907} and selectively freezing pre-trained parameters~\citep{kirkpatrick2017overcoming,lee2019would,guo2019spottune,ramasesh2020anatomy,liu2021autofreeze, royer2020flexible, eastwood2021source, evci2022head2toe, eastwood2022unit, cohen2022my, touvron2022three,lee2022surgical,kumar2022sgdfinetuning}. 
However, as pre-trained models are fine-tuned for a specific distribution, their effective robustness decreases at convergence~\citep{andreassen2021evolution}.
We introduce a transfer learning framework that preserves the robustness of the pre-trained model while adapting to new tasks.

\textbf{AutoML and bi-level optimization.}
Our work leverages high-level ideas from the broader literature on meta-learning and hyperparameter optimization.
Such methods have proposed to optimize different parts of the training pipeline, including general hyperparameters \citep{hutter2011sequential,bergstra2012random,feurer2015efficient,li2017hyperband,li2018massively},
network architectures \citep{zoph2016neural,zoph2018learning,liu2018darts,real2019regularized,xu2019pc}, 
augmentation policies \citep{cubuk2019autoaugment,lim2019fast,hataya2020faster,cubuk2020randaugment}, 
optimizers \citep{bengio2013optimization,andrychowicz2016learning,wichrowska2017learned,metz2022velo,chen2023symbolic}, 
and objective functions~\citep{yu2018one,kirsch2019improving,oh2020discovering,bechtle2021meta}.
%%CF.11.15: there are also works that optimize loss functions, and it would be good to cite them. Bechtle et al. is one. We used a learned loss in one-shot imitation from human videos. Maybe we used one in the ARM paper too? Can look at the papers that cite bechtle et al. 
However, most of these works optimize for generalization within the training distribution and do not consider robustness to distribution shifts.
Existing works that optimize a training procedure for OOD generalization consider a structured few-shot adaptation setting \citep{li2018learning,zhang2021adaptive}, limiting their scalability to large datasets.
\citet{tian2023trainable} learn layer-specific regularization constraints to improve OOD generalization; however, they do not learn a fine-tuning objective.
% For fine-tuning \cite{Li2020Rethinking} \cite{plested2021rethinking}
% \cite{bai2021ood} investigate neural architecture search for OOD generalization. They optimize architectures based on their performance on synthetically generated OOD data by jointly optimizing an OOD data generator and architecture search.
% \cite{zhang2023hypertime} use hyperparameter optimization to improve the robustness of models to temporal distribution shifts. 
% They perform hyperparameter tuning with a lexicographic preference across different objectives that balances average and worst-case validation losses from different time periods.
% Notably, these works do not consider the transfer learning setting and do not learn the loss.
% Our work learns how to best adapt a foundation model to a new task by optimizing hyperparameters on an OOD validation set.

\textbf{Out-of-distribution generalization.}
Maintaining good performance on data that deviates from the training distribution is crucial in many real-world applications, where models may face data from unfamiliar environments~\citep{hendrycks2019robustness,geirhos2020shortcut,gulrajani2020search,koh2021wilds}.
Numerous studies have investigated how to ensure robustness to various distribution shifts~\citep{tzeng2014deep,byrd2019effect,hendrycks2019using,arjovsky2019invariant,salman2020adversarially,liu2021just,wiles2021fine, andreassen2021evolution,creager2021environment,lee2022diversify}.
Some works have shown that despite the myriad of ways in which data distributions can change, naturally occurring distribution shifts have a surprisingly predictable effect on model performance~\citep{taori2020measuring,miller2021accuracy,baek2022agreement}, suggesting that it may be possible to \textit{learn} how to be robust to unseen natural distribution shifts.
Similar to our work, \citet{goyal2022test} meta-learn an objective, but for test-time adaptation instead of fine-tuning.
% \citet{goyal2022test} meta-learn an objective for test-time adaptation.
% However, \ours{} focuses on the fine-tuning stage before deployment and does not assume access to test data.
% \ours{} improves generalization to novel distribution shifts after fine-tuning using only a small OOD validation set.
% \ours{} uses post-adaptation performance on a small OOD validation set that is not from the test OOD distributions to learn a robust fine-tuning procedure.
Benchmarks for OOD generalization, such as DomainBed~\citep{gulrajani2020search} and WILDS~\citep{koh2021wilds}, have discussed data assumptions for dealing with distribution shifts, and suggested that an OOD validation set can be a useful signal for hyperparameter optimization and model selection.
\ours{} leverages this signal much more directly than existing works by learning an objective for fine-tuning.
% have been proposed to evaluate and improve OOD generalization.
% Prior works on OOD generalization select models and hyperparameters based on performance on a held-out domain or OOD validation set \citep{gulrajani2020search,koh2021wilds}.
% In contrast, \ours{} focuses on learning a good objective function for robust fine-tuning, which results in more nuanced adaptation and better OOD generalization.

%%CF.11.15: Ideally, it should be obvious after reading how our work is distinct from these prior works. But, right now, this isn't really conveyed.
%%CF.11.15: Also, are you citing the CMU paper that meta-learned a loss for test-time training? That seems fairly relevant from a methodological point of view (though obviously has some key differences that would also be good to convey)

% Neural networks often fail to generalize to data outside the training distribution~\citep{hendrycks2019robustness,geirhos2020shortcut,li2021measuring}, limiting their applicability in many real-world settings.
% Many works have proposed methods to improve OOD generalization by incorporating additional information~\citep{tzeng2014deep,ganin2016domain,arjovsky2019invariant,sagawa2019distributionally,nam2020learning,creager2021environment,liu2021just,zhang2022contrastive}.
% We focus on the transfer learning setting, where striking the right balance between the pre-trained model and new task-specific data is crucial for OOD generalization.
% We assume access to a small OOD validation set, which is not large enough to effectively fine-tune a model, but can serve as a useful signal for hyperparameter optimization.
% Other research has delved into model behaviors under distribution shifts, showing that a model's accuracy on a reference distribution typically aligns with its robustness to distribution shifts~\cite{taori2020measuring,miller2021accuracy,baek2022agreement}.
% unused robustness citations
% CLIP~\citep{radford2021learning}
% accuracy-on-the-line, effective robustness~\citep{miller2021accuracy}
% Contrastive-like fine-tuning objective for low-shot robustness~\citep{goyal2022finetune}
% Inconsistent results in low shot settings\citep{singh2023benchmarking}
% data assumptions for spurious correlation
% \cite{liu2021just} notes that tuning for WGA assumes group labels
% \cite{bao2022learning} introduces a simple baseline

% Robust fine-tuning
\textbf{Robust fine-tuning.}
% This robustness implies that such models learn features that serve as a valuable prior for a range of tasks. 
% The challenge of fine-tuning foundation models while maintaining accuracy under distribution shifts is increasingly crucial as foundation models become more prevalent yet remains an open problem~\citep{andreassen2021evolution,bommasani2021opportunities}.
% Existing robustness interventions fail to offer uniform improvements over distribution shifts where zero-shot models perform well~\cite{taori2020measuring}.
% Motivated by the fact that foundation models often achieve higher OOD performance than naively fine-tuned models, 
Foundation models trained on massive datasets encode a broad range of general knowledge, enabling robust performance across various data distributions, including OOD scenarios~\citep{radford2021learning,bommasani2021opportunities}.
While in principle, foundation models should serve as a useful prior for further fine-tuning, empirical evidence shows that fine-tuning foundation models on a new task often leads to a significant drop in OOD performance~\citep{andreassen2021evolution}.
% As foundation models become more prevalent, adapting them to new tasks while maintaining or improving their performance under distribution shifts is an increasingly crucial challenge.
Recent works have proposed modifications to the basic fine-tuning procedure to improve OOD generalization~\citep{wortsman2022robust,kumar2022fine,wortsman2022model,goyal2022finetune,mukhoti2023fine}.
% Perhaps separate into (prompt tuning, Adapters, ensembles)
Instead of hand-designing a regularization technique, we propose a data-driven approach to \textit{learn} a more nuanced fine-tuning procedure. 
In fact, some prior works~\citep{xuhong2018explicit,lee2022surgical,goyal2022finetune} can be seen as \textit{special cases} of \ours{} since our hyperparameter search space encompasses these fine-tuning algorithms.
Our experiments in~\cref{sec:results} demonstrate that \ours{} consistently outperforms prior robust fine-tuning methods on OOD data.
%%CF.11.15: maybe also mention that we empirically improve over some of these prior methods? x
% \citep{pham2021combined}

%%CF.11.15: This paper would be good to add: https://arxiv.org/pdf/2211.16175v1.pdf

% % Learned optimizers
% Early~\citep{bengio2013optimization,runarsson2000evolution}
% Modern, RNN optimizer, full backprop~\citep{andrychowicz2016learning}
% Learned optimizers that scale and generalize~\citep{wichrowska2017learned}
% A closer look at learned optimizers~\citep{harrison2022closer}
% VeLO~\citep{metz2022velo}
% Lion, symbolic discovery~\citep{chen2023symbolic}
% learned optimizer with input noise robustness~\citep{metz2019using}
% Learned loss functions~\citep{XXX} or learning rates~\citep{XXX}


% The complications usually associated with in-distribution generalization are magnified when testing on data outside the training distribution.
% Many works focus on optimizing in-distribution (ID) performance, assuming that it will naturally translate to good OOD performance.
% However, recent findings indicate a more complex relationship between ID and OOD performance.
% For example, \citep{teney2022id} observes that ID and OOD performance are sometimes inversely correlated.
% Similarly, \citep{yang2023change} shows that the choice of evaluation metric for model selection can significantly impact performance under distribution shift, particularly worst-group accuracy.
% This aligns with distribution-shift benchmarks that suggest tuning hyperparameters on OOD data, such as DomainBed \citep{gulrajani2020search} and WILDS \citep{koh2021wilds}.
%accuracy-on-the-line ~\citep{miller2021accuracy}.




==> arxiv/sections/results.tex <==
\input{tables/iwildcam_sota.tex}

In this section, we present the main experimental findings for \ours{}. 
We show that \ours{} improves OOD generalization on nine distribution shifts.
We present additional results in the low-data and IID transfer learning regimes in \cref{sec:few-shot} and \cref{sec:transfer-learning}.
These findings highlight the effectiveness of \ours{} for robust fine-tuning in a variety of settings.
Finally, we investigate whether the hyperparameters learned by \ours{} transfer across fine-tuning datasets, and analyze the choice of OOD validation dataset.

\input{tables/fmow_sota.tex}

\begin{figure*}[t]
\vspace{-1mm}
\centering 
\includegraphics[width=1.0\linewidth]{figures/scatter_plot_new.pdf}
\vspace{-5mm}
\caption{\ours{} outperforms existing methods, both with and without weight ensembling~\citep{wortsman2022robust}.
Here, we show the ID-OOD performance curves obtained by linearly interpolating the fine-tuned model weights with the zero-shot weights.
}
\label{fig:effective-robustness-plots}
\end{figure*}

\begin{table*}[t]
\vspace{0mm}
    \centering
    \input{tables/big_table_arxiv}
\end{table*}

\input{tables/hparam_transfer.tex}
\input{tables/validation_sets.tex}

% Tables for ablations section; moved here to avoid page break


\subsection{Distribution Shifts}

\textbf{\ours{} improves OOD generalization.} 
We evalute \ours{} on three common robust fine-tuning benchmarks: ImageNet, WILDS-FMoW, and WILDS-iWildCam. 
This evaluation includes diverse distribution shift conditions including subpopulation and domain shifts.
ID and OOD performance reported in~\cref{tab:big_distribution_shift_table} show that \ours{} consistently outperforms existing methods for robust fine-tuning in OOD metrics.
Furthermore, these gains are maintained when ensembling initial and fine-tuned models, suggesting that the benefits from \ours{} are complementary to that of ensembling~\citep{wortsman2022robust,wortsman2022model}.
% In these diverse distribution shifts including subpopulation and domain shifts, \ours{} consistently
We show additional experiments on CIFAR-10 and related distribution shifts in~\cref{tab:cifar10}, which show the same conclusion.
% \cref{tab:big_distribution_shift_table} contains results on ImageNet, WILDS-FMoW, and WILDS-iWildCam; results on CIFAR-10 are in ~\cref{tab:cifar10}.
% \ours{} consistently outperforms all baselines on OOD distributions.
% These gains are maintained when ensembling zero-shot and fine-tuned models.

\textbf{State-of-the-art performance on iWildCam and FMoW.}
To further assess whether the robustness gains from \ours{} scale to larger foundation models, we evaluate \ours{} with a \texttt{ViT-L/14@336px} model, following the largest scale experiment in \citet{goyal2022finetune}.
Results in \cref{tab:sota_iwild} show that \ours{} improves upon the prior state-of-the-art method, FLYP \citep{goyal2022finetune}, by $6.0\%$ in OOD macro-F1.
Furthermore, on WILDS-FMoW~\cref{tab:sota_fmow}, \ours{} outperforms a Transformer-specific parameter freezing method~\citep{kumar2022sgdfinetuning}, the prior state-of-the-art, by $1.5\%$ in OOD worst-region accuracy.
Additionally, \ours{} outperforms the compute-intensive Model Soups~\citep{wortsman2022model} on both benchmarks; this method ensembles more than $70$ models fine-tuned with different augmentations and hyperparameters.
% On both benchmarks, \ours{} additionally outperforms the compute-intensive Model Soups \citep{wortsman2022model}, which ensembles more than 70 models fine-tuned with LP-FT and different augmentations and hyperparameters. 


\subsection{Few-Shot Classification}
\label{sec:few-shot}

% \input{tables/fewshot_binary.tex}

Many real-world applications have limited labeled data for fine-tuning.
Thus, few-shot classification serves as an important benchmark for fine-tuning.
Few-shot binary classification is a particularly challenging task for adaptation, given the small number of training examples.
We evaluate on 4, 16, and 32 shot binary classification tasks from the PatchCamelyon and Rendered-SST2 datasets, following \citet{radford2021learning} and \citet{goyal2022finetune}.
PatchCamelyon contains digital pathology images for the detection of metastatic tissue.
Rendered-SST2 focuses on optical character recognition for classifying text sentiment.

\ours{} demonstrates strong generalization capabilities given limited data, outperforming all baselines in \cref{tab:fewshot-binary-classification}. 
For example, \ours{} outperforms FLYP by $3.7\%$ and full fine-tuning by $3.9\%$ in a challenging 4-shot classification task on Rendered-SST2.


\begin{figure*}
\vspace{-1mm}
\begin{minipage}[b]{0.72\textwidth}
\centering
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{3}{c}{PatchCamelyon} & \multicolumn{3}{c}{SST2} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
$k$ (shots) & 4 & 16 & 32 & 4 & 16 & 32 \\
\midrule
Zeroshot & 56.5 (-) & 56.5 (-) & 56.5 (-) & 60.5 (-) & 60.5 (-) & 60.5 (-) \\
LP & 60.4 (4.0) & 64.4 (3.7) & 67.0 (4.4) & 60.8 (1.8) & 61.9 (1.4) & 62.9 (1.3) \\
FT & 63.1 (5.5) & 71.6 (4.6) & 75.2 (3.7) & 61.1 (0.7) & 62.4 (1.6) & 63.4 (1.9) \\
LP-FT & 62.7 (5.3) & 69.8 (5.3) & 73.9 (4.6) & 60.9 (2.4) & 62.9 (1.9) & 63.6 (1.4) \\
FLYP & 66.9 (5.0) & 74.5 (2.0) & 76.4 (2.4) & 61.3 (2.7) & 65.6 (2.1) & 68.0 (1.7) \\
\midrule
% \rowcolor[gray]{0.8}
\oursbf{} & \textbf{68.1 (5.1)} & \textbf{76.8 (2.9)} & \textbf{79.5 (2.0)} & \textbf{65.0 (3.8)} & \textbf{67.5 (1.1)} & \textbf{69.0 (1.1)} \\
\bottomrule
\end{tabular}
}
\vspace{-2mm}
\caption{In binary few-shot classification, \ours{} outperforms existing robust fine-tuning methods. 
\ours{} outperforms FLYP by $3.1\%$ and full fine-tuning by $4.3\%$ in 32-shot classification on PatchCamelyon.
}
\label{tab:fewshot-binary-classification}
\end{minipage}
\hfill
\begin{minipage}[b]{0.26\textwidth}
\centering
% \begin{table} \centering
\begin{tabular}{lcc}
\toprule
Examples & ID & OOD \\
\midrule
% FLYP          & 52.2    & 35.6     \\
200          & 48.9    & 37.2     \\
1000         & 51.0    & \textbf{38.3} \\
5000         & 50.4    & 38.0     \\
10000        & 48.9    & 37.8     \\
\bottomrule
\end{tabular}
\caption{
\label{tab:val-set-size}
\textbf{Effect of val set size.} 
Performance of \ours{} on iWildCam with varying validation set sizes. Increasing size beyond $1000$ shows minimal additional benefits.}
% \end{table}
\end{minipage}
\end{figure*}

% \subsection{Transfer Learning}

% In standard transfer learning settings, where no distribution shifts exist between train and test data, \ours{} shows strong performance.
% The primary goal here is to achieve strong in-distribution (ID) performance on the test set.
% In this setting, \ours{} uses a small ID validation set to optimize hyperparameters.

% We compare \ours{} against other baselines on several transfer learning datasets: CalTech-101, StanfordCars, and Flowers-102 in \cref{tab:transfer_learning}. 
% \ours{} matches or outperforms all baselines on 2 of the 3 transfer learning datasets, outperforming FLYP by $1.4\%$ on CalTech-101.


\subsection{Transfer Learning}
\label{sec:transfer-learning}

We additionally evaluate \ours{} in a standard transfer learning setting, where the evaluation data is drawn from the same distribution as both the training and validation data.
We compare \ours{} against other fine-tuning methods on several transfer learning datasets: CalTech-101, Stanford Cars, and Flowers-102.
Results in~\cref{tab:transfer_learning} demonstrate that \ours{} is competitive with these baselines, but the advantages from learning an objective are less pronounced compared to previous experiments.
This indicates that problem-specific learned fine-tuning objectives are most helpful in settings with high underspecification such as OOD evaluation conditions or few-shot learning, confirming our initial intuition in~\cref{sec:method}.

% In IID transfer learning settings where no distribution shifts exist between train and test data, \ours{} shows strong performance when using a small ID validation set to learn the objective and hyperparameters.
% The primary goal here is to achieve strong in-distribution (ID) performance on the test set.
% % In this setting, \ours{} uses a small ID validation set to optimize hyperparameters.
% We compare \ours{} against other baselines on several transfer learning datasets: CalTech-101, StanfordCars, and Flowers-102 in \cref{tab:transfer_learning}. 
% \ours{} matches or outperforms all baselines on 2 of the 3 transfer learning datasets, outperforming FLYP by $1.4\%$ on CalTech-101.


==> arxiv/tables/alg.tex <==
\newcommand{\algcomment}[1]{%
\hfill {\raggedleft\textcolor{gray!60}{// #1}\par}
}
\begin{algorithm}[t]
\caption{\label{alg:hyperopt} \ours{}}
\begin{algorithmic}[1]
    \REQUIRE Hyperparameter Optimizer (HPO)
    \REQUIRE ID Training Data $\Dtr$, OOD Validation Data $\Dval$
    \FOR{$\phi \leftarrow \text{HPO.Sample}()$}
        \STATE $f_{ft} \leftarrow \LA(\Dtr, \mathcal{L}_\phi)$ \algcomment{Short fine-tuning run with sampled loss}
        \STATE $p \leftarrow \mathrm{Perf}(f_{ft}, \Dval)$ \algcomment{Evaluation on OOD Val set}
        % \STATE $\mathrm{HPO}.\mathrm{Update}(\phi, p)$ \algcomment{HPO Update}
    \ENDFOR
    \STATE $\phi^* \leftarrow \mathrm{HPO}.\mathrm{Best}()$ \algcomment{Get best hyperparameters}
    \STATE $f^* \leftarrow \LA(\Dtr, \mathcal{L}_{\phi^*})$ \algcomment{Fine-tune with loss $\mathcal{L}_{\phi^*}$}
    \STATE \textbf{Return} $f^*$
\end{algorithmic}
\end{algorithm}


==> arxiv/tables/big_table.tex <==
\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{@{}ccccccccc@{}}
\toprule
& \multicolumn{4}{c}{iWILDCam} & \multicolumn{4}{c}{FMoW} \\ \cmidrule(l){2-9} 
& \multicolumn{2}{c}{Without Ensembling} & \multicolumn{2}{c|}{With Ensembling} & \multicolumn{2}{c}{Without Ensembling} & \multicolumn{2}{c}{With Ensembling} \\ 
\cmidrule(lr){2-3}  \cmidrule(lr){4-5}  \cmidrule(lr){6-7}  \cmidrule(lr){8-9} 
\multirow{-3}{*}{Methods} & ID & OOD & ID & \multicolumn{1}{c|}{OOD} & ID & OOD & ID & OOD \\ \midrule
Zeroshot & 8.7 (-) & 11.0 (-) & 8.7 (-) & \multicolumn{1}{c|}{11.0 (-)} & 20.4 (-) & 18.7 (-) & 20.4 (-) & 18.7 (-) \\
LP & 44.5 (0.6) & 31.1 (0.4) & 45.5 (0.6) & \multicolumn{1}{c|}{31.7 (0.4)} & 48.2 (0.1) & 30.5 (0.3) & 48.5 (0.1) & 30.7 (0.3) \\
FT & 48.1 (0.5) & 35.0 (0.5) & 48.1 (0.5) & \multicolumn{1}{c|}{35.0 (0.5)} & 68.5 (0.1) & 39.2 (0.7) & 68.5 (0.1) & 39.2 (0.7)\\
L2-SP & 48.6 (0.4) & 35.3 (0.3) & 48.6 (0.4) & \multicolumn{1}{c|}{35.3 (0.3)} & 68.6 (0.1) & 39.4 (0.6) & 68.6 (0.1) & 39.4 (0.6) \\
LP-FT & 49.7 (0.5) & 34.7 (0.4) & 50.2 (0.5) & \multicolumn{1}{c|}{35.7 (0.4)} & 68.4 (0.2) & 40.4 (1.0) & 68.4 (0.2) & 40.4 (1.0) \\
FLYP & \textbf{52.2 (0.6)} & 35.6 (1.2) & \textbf{52.5 (0.6)} & \multicolumn{1}{c|}{37.1 (1.2)} & \textbf{68.6 (0.2)} & 41.3 (0.8) & \textbf{69.0 (0.1)} & 41.9 (0.7) \\ \midrule
\oursbf{} & 51.0 (0.5) & \textbf{38.3 (0.5)} & 51.3 (0.5)  & \textbf{39.3 (0.5)} & 67.1 (0.3) & \textbf{42.3 (0.5)} & 67.1 (0.3) & \textbf{42.3 (0.5)} \\
\bottomrule
\end{tabular}
}
\caption{
\ours{} outperforms all baselines both with and without ensembling.
Without ensembling, \ours{} improves OOD performance by $3.7\%$ on WILDS-iWildCam and $6.1\%$ on WILDS-FMoW, respectively. 
On WILDS-iWildCam, these improvements are preserved with ensembling, leading to an increase of $2.2\%$ in OOD macro F1.
}
\label{tab:big_distribution_shift_table}

==> arxiv/tables/big_table_arxiv.tex <==
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}ccccc|cccc|cc@{}}
\toprule
& \multicolumn{4}{c|}{ImageNet} & \multicolumn{4}{c|}{iWILDCam} & \multicolumn{2}{c}{FMoW} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-11}
& \multicolumn{2}{c}{Without Ensembling} & \multicolumn{2}{c|}{With Ensembling} & \multicolumn{2}{c}{Without Ensembling} & \multicolumn{2}{c|}{With Ensembling} & \multicolumn{2}{c}{Without Ensembling} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
Methods & ID & OOD & ID & OOD & ID & OOD & ID & OOD & ID & OOD \\
\midrule
Zeroshot & 68.3 (-) & 58.7 (-) & 68.3 (-) & 58.7 (-) & 8.7 (-) & 11.0 (-) & 8.7 (-) & 11.0 (-) & 20.4 (-) & 18.7 (-) \\
LP & 79.9 (0.0) & 57.2 (0.0) & 80.0 (0.0) & 58.3 (0.0) & 44.5 (0.6) & 31.1 (0.4) & 45.5 (0.6) & 31.7 (0.4) & 48.2 (0.1) & 30.5 (0.3) \\
FT & 81.4 (0.1) & 54.8 (0.1) & 82.5 (0.1) & 61.3 (0.1) & 48.1 (0.5) & 35.0 (0.5) & 48.1 (0.5) & 35.0 (0.5) & 68.5 (0.1) & 39.2 (0.7) \\
L2-SP & 81.6 (0.1) & 57.9 (0.1) & 82.2 (0.1) & 58.9 (0.1) & 48.6 (0.4) & 35.3 (0.3) & 48.6 (0.4) & 35.3 (0.3) & 68.6 (0.1) & 39.4 (0.6) \\
LP-FT & 81.8 (0.1) & 60.5 (0.1) & 82.1 (0.1) & 61.8 (0.1) & 49.7 (0.5) & 34.7 (0.4) & 50.2 (0.5) & 35.7 (0.4) & 68.4 (0.2) & 40.4 (1.0) \\
FLYP & 82.6 (0.0) & 60.2 (0.1) & 82.9 (0.0) & 63.2 (0.1) & 52.2 (0.6) & 35.6 (1.2) & 52.5 (0.6) & 37.1 (1.2) & 68.6 (0.2) & 41.3 (0.8) \\
\midrule 
\ours{} & 81.8 (0.1) & \textbf{61.5 (0.1)} & 82.4 (0.1) & \textbf{64.3 (0.1)} & 51.0 (0.5) & \textbf{38.3 (0.5)} & 51.3 (0.5)  & \textbf{39.3 (0.5)} & 67.1 (0.3) & \textbf{42.3 (0.5)} \\
\bottomrule
\end{tabular}
}
\caption{
\ours{} outperforms all baselines both with and without ensembling.
Without ensembling, \ours{} improves OOD performance by $1.3\%$ on ImageNet, $2.7\%$ on WILDS-iWildCam, and $1.0\%$ on WILDS-FMoW. 
These improvements are preserved with weight ensembling.
}
\label{tab:big_distribution_shift_table}


==> arxiv/tables/cifar.tex <==
\begin{table}
\centering
% \resizebox{0.95\linewidth}{!}{
\begin{tabular}{ccc}
\toprule
Method & CIFAR-10.1 & CIFAR-10.2 \\
\midrule
Zero-shot & 92.5 & 88.8 \\
Fine-tuning & 95.9 & 91.3 \\
% \rowcolor[gray]{0.8}
\oursbf & \textbf{97.5} & \textbf{93.5} \\
\midrule
% WiSE-FT ($\alpha=0.5$) & 97.6 & 93.4 \\
WiSE-FT (best $\alpha$) & 98.0 & 94.4 \\
% \rowcolor[gray]{0.8}
\oursbf{} (best $\alpha$) & \textbf{98.3} & \textbf{95.0} \\
\bottomrule
\end{tabular}
% }
\caption{\textbf{Evaluation on CIFAR-10 distribution shifts.} \ours{} outperforms fine-tuning by $2.2\%$ on CIFAR-10.2 and by $1.4\%$ on CIFAR-10.1, using only 100 samples from CIFAR-10-C.
\ours{} additionally outperforms WiSE-FT with weight ensembling.}
\label{tab:cifar10}
\vspace{-5.0pt}
\end{table}

==> arxiv/tables/fewshot_binary.tex <==
\begin{table*}[t!]
\centering
% \resizebox{1.03\linewidth}{!}{
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{3}{c}{PatchCamelyon} & \multicolumn{3}{c}{SST2} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
$k$ (shots) & 4 & 16 & 32 & 4 & 16 & 32 \\
\midrule
Zeroshot & 56.5 (-) & 56.5 (-) & 56.5 (-) & 60.5 (-) & 60.5 (-) & 60.5 (-) \\
LP & 60.4 (4.0) & 64.4 (3.7) & 67.0 (4.4) & 60.8 (1.8) & 61.9 (1.4) & 62.9 (1.3) \\
FT & 63.1 (5.5) & 71.6 (4.6) & 75.2 (3.7) & 61.1 (0.7) & 62.4 (1.6) & 63.4 (1.9) \\
LP-FT & 62.7 (5.3) & 69.8 (5.3) & 73.9 (4.6) & 60.9 (2.4) & 62.9 (1.9) & 63.6 (1.4) \\
FLYP & 66.9 (5.0) & 74.5 (2.0) & 76.4 (2.4) & 61.3 (2.7) & 65.6 (2.1) & 68.0 (1.7) \\
\midrule
% \rowcolor[gray]{0.8}
\oursbf{} & \textbf{68.1 (5.1)} & \textbf{76.8 (2.9)} & \textbf{79.5 (2.0)} & \textbf{65.0 (3.8)} & \textbf{67.5 (1.1)} & \textbf{69.0 (1.1)} \\
\bottomrule
\end{tabular}
% }
\vspace{-2mm}
\caption{In binary few-shot classification, \ours{} outperforms existing robust fine-tuning methods. 
\ours{} outperforms FLYP by $3.1\%$ and full fine-tuning by $4.3\%$ in 32-shot classification on PatchCamelyon.
}
\label{tab:fewshot-binary-classification}
\end{table*}

==> arxiv/tables/fmow_sota.tex <==
\begin{table}[t]
\centering
\begin{tabular}{@{}llcc@{}}
\toprule
Method & Architecture & ID & OOD \\
\midrule
Group DRO & DenseNet121 & 51.2 (0.4) & 31.1 (1.7) \\
LISA & DenseNet121 & 52.8 (1.2) & 35.5 (0.8) \\
ERM w/ aug & DenseNet121 & 55.5 (0.4) & 35.7 (0.3) \\
% DFR & DenseNet121 & 42.8 (0.4) & 53.4 (0.4) \\
DFR & DenseNet121 & 53.4 (0.4) & 42.8 (0.4) \\
ERM & ViTL & 66.9 (0.2) & 46.1 (0.6) \\
Model Soups & ViTL & 69.5 (0.1) & 47.6 (0.3) \\
Freeze-Embed & ViTL-336px & 68.3 (0.4) & 50.3 (1.1) \\
\midrule
\oursbf{} & ViTL-336px & 72.1 (0.1) & \textbf{51.8 (0.4)} \\
\bottomrule
\end{tabular}
\caption{
    \textbf{FMoW results.}
    \ours{} with weight ensembling attains state-of-the-art OOD performance on the WILDS-FMoW benchmark with a \texttt{ViT-L/14-336px} backbone, surpassing all prior entries on the WILDS leaderboard \citep{koh2021wilds}.}
\label{tab:sota_fmow}
\vspace{-3mm}
\end{table}

==> arxiv/tables/hparam_transfer.tex <==
\begin{table}[t!]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{2}{c}{MNIST} & \multicolumn{2}{c}{CIFAR10.2} & \multicolumn{2}{c}{CIFAR10.1} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
Method & ID & OOD & ID & OOD & ID & OOD \\ 
\midrule
FT & 99.8 & 62.3 & 97.9 & 96.2 & 98.3 & 93.4 \\ 
\oursbf{} & 99.8 & 61.1 & 98.2 & 96.3 & 98.4 & 93.4 \\
\bottomrule
\end{tabular}
}
\vspace{-2mm}
\caption{
% Finetuning with hyperparameters learned on the CIFAR-10 and CIFAR-10-C distributions.
Performance comparison of models fine-tuned on new distributions with hyperparameters learned by \ours{} on a different dataset, CIFAR-10.
Hyperparameters transfer better to datasets that are more similar to the original fine-tuning distribution.
}
\label{tab:hparam-transfer}
\end{table}


==> arxiv/tables/iwildcam_sota.tex <==
% \begin{table}[t]
% \centering
% \resizebox{0.99\linewidth}{!}{%
% \begin{tabular}{@{}cccc@{}}
% \toprule
% \multicolumn{1}{l}{} & Architecture & ID                  & OOD                 \\ \midrule
% ABSGD                & ResNet50     & 47.5 (1.6)          & 33.0 (0.6)          \\ 
% ERM                  & PNASNet      & 52.8 (1.4)          & 38.5 (0.6)          \\
% ERM                  & ViTL         & 55.8 (1.9)          & 41.4 (0.5)          \\
% Model Soups          & ViTL         & 57.6 (1.9)          & 43.3 (1.0)           \\
% FLYP                 & ViTL-336px   & 59.9 (0.7) & 46.0 (1.3) \\
% \midrule
% % \oursbf{}            & ViTL-336px   & 58.2 (1.0) & \textbf{50.6 (0.5)} \\
% \oursbf{}            & ViTL-336px   & \textbf{63.5 (0.5)} & \textbf{52.0 (0.4)} \\ % from our official WILDS submission
% \bottomrule
% \end{tabular}
% }
% \caption{\ours{} with weight ensembling attains state-of-the-art OOD performance on the WILDS-iWildCam benchmark with a \texttt{ViT-L/14-336px} backbone, surpassing the top five entries on the leaderboard \citep{koh2021wilds}. We observe similar performance gains by \ours{} using a smaller \texttt{ViT-B/16} architecture in \cref{tab:big_distribution_shift_table}.}
% \label{tab:sota_iwild}
% \end{table}

\begin{table}[t]
\centering
\begin{tabular}{@{}llcc@{}}
\toprule
Method & Architecture & ID & OOD \\
\midrule
Group DRO & ResNet50 & 37.5 (1.9) & 23.8 (2.0) \\
ABSGD & ResNet50 & 47.5 (1.6) & 33.0 (0.6) \\
Copy-Paste & ResNet50 & 50.2 (1.6) & 36.5 (0.9) \\
ERM & PNASNet & 52.8 (1.4) & 38.5 (0.6) \\
ERM & ViTL & 55.8 (1.9) & 41.4 (0.5) \\
Model Soups & ViTL & 57.6 (1.9) & 43.3 (1.0) \\
FLYP & ViTL-336px & 59.9 (0.7) & 46.0 (1.3) \\
\midrule
\oursbf{} & ViTL-336px & 63.5 (0.5) & \textbf{52.0 (0.4)} \\
\bottomrule
\end{tabular}
\caption{
    \textbf{iWildCam results.}
    \ours{} with weight ensembling attains state-of-the-art OOD performance on the WILDS-iWildCam benchmark with a \texttt{ViT-L/14-336px} backbone, surpassing all prior entries on the WILDS leaderboard \citep{koh2021wilds}.}
\label{tab:sota_iwild}
\vspace{-3mm}
\end{table}

==> arxiv/tables/layerwise.tex <==
% \begin{table}
% \begin{minipage}{\linewidth}
% \centering
% \begin{tabular}{ccc}
% \toprule
% \multicolumn{3}{c}{iWildCam} \\
% \midrule 
% Method & ID & OOD \\
% \midrule
% \ours & \textbf{51.0} & \textbf{38.3} \\
% Layerwise \ours & 47.8 & 34.6 \\
% \bottomrule
% \end{tabular}
% \end{minipage}
% \caption{\ours{} yields better ID and OOD performance than its variant with per-layer learning rates, weight decays, and L1/L2 distances to pretrained parameters, indicating that more expressive hyperparameter spaces overfit to the validation set, degrading performance.}
% \label{tab:expressivity}
% \end{table}

\centering
\begin{tabular}{ccc}
\toprule
\multicolumn{3}{c}{iWildCam} \\
\midrule 
Method & ID & OOD \\
\midrule
\ours & \textbf{51.0} & \textbf{38.3} \\
Layerwise \ours & 47.8 & 34.6 \\
\bottomrule
\end{tabular}
\caption{\textbf{Expressivity of the \ours{} search space.} \ours{} results in better performance than its layerwise variant with per-layer learning rates, weight decays, and L1/L2 distances to pretrained parameters. Evaluation is on the iWildCam benchmark. This suggests that more expressive hyperparameter spaces overfit to the validation set, degrading performance.}
\label{tab:expressivity}
\vspace{-5.0pt}

==> arxiv/tables/transfer_learning.tex <==
% \begin{table}[h]
% \centering
% \begin{tabular}{lcccccc}
% \toprule
% Methods & PCAM & CalTech & Cars & Flowers & ImageNet & iWILD \\
% \midrule
% Zeroshot & 56.49 (-) & 87.7 (-) & 64.4 (-) & 71.2 (-) & 68.3 (-) & 8.7 (-) \\
% LP & 82.6 (0.1) & 94.8 (0.0) & 83.1 (0.0) & 95.9 (0.0) & 79.9 (0.0) & 44.5 (0.6) \\
% FT & 89.1 (1.3) & 97.2 (0.1) & 84.4 (0.3) & 90.4 (0.5) & 81.4 (0.1) & 48.1 (0.5) \\
% LP-FT & 89.0 (0.6) & 96.9 (0.6) & 89.4 (0.1) & 97.9 (0.1) & 81.8 (0.1) & 49.7 (0.5) \\
% FLYP & 90.3 (0.3) & 97.6 (0.1) & 89.6 (0.3) & 97.7 (0.1) & 82.6 (0.0) & 52.2 (0.6) \\
% \midrule
% \oursbf{} & x.x (x.x) & \textbf{99.0 (0.2)} & x.x (x.x) & x.x (x.x) & x.x (x.x) & x.x (x.x) \\
% \bottomrule
% \end{tabular}
% \caption{In addition to enhancing robustness, \ours{} improves in-distribution performance after fine-tuning.}
% \label{tab:transfer_learning}
% \end{table}

\begin{table*}[t!]
\vspace{-2mm}
\centering
% \resizebox{0.95\linewidth}{!}{
\begin{tabular}{lccc}
\toprule
Methods & CalTech-101 & Stanford Cars & Flowers-102 \\
\midrule
Zeroshot & 87.7 (-) & 64.4 (-) & 71.2 (-) \\
LP & 94.8 (0.0) & 83.1 (0.0) & 95.9 (0.0) \\
FT & 97.2 (0.1) & 84.4 (0.3) & 90.4 (0.5) \\
LP-FT & 96.9 (0.6) & 89.4 (0.1) & \textbf{97.9 (0.1)} \\
FLYP & 97.6 (0.1) & \textbf{89.6 (0.3)} & 97.7 (0.1) \\
\midrule
% \rowcolor[gray]{0.8}
\oursbf{} & \textbf{99.0 (0.1)} & \textbf{89.6 (0.2)} & 97.6 (0.2) \\
\bottomrule
\end{tabular}
% }
\vspace{-2mm}
\caption{
\textbf{\ours{} can lead to improvements in IID transfer learning.} In addition to enhancing OOD generalization, \ours{} can improve performance in IID transfer learning settings when using an ID validation set to learn the objective and hyperparameters..
% , where there is no distribution shift. 
% Here, \ours{} uses ID validation examples to learn the objective and hyperparameters.
% \ours{} outperforms baselines on CalTech-101 and performs similarly to the best baseline on Stanford Cars and Flowers-102.
}
\label{tab:transfer_learning}
\end{table*}


==> arxiv/tables/validation_sets.tex <==
\begin{table}[t!]
\centering
    \begin{tabular}{cccc}
    \toprule
    Validation Dataset & CIFAR-10.1 & CIFAR-10.2 \\
    \midrule
    CIFAR-10-C & 97.4 (0.2) & 93.5 (0.2) \\
    CIFAR-10 & 96.9 (0.2) & 93.2 (0.1) \\
    CIFAR-10.1 & 96.8 (0.3) & 92.8 (0.2) \\
    CIFAR-10.2 & 96.7 (0.5) & 93.8 (0.0) \\
    \bottomrule
    \end{tabular}
    % }
\vspace{-2mm}
    \caption{
    \label{tab:varying_validation_sets}
        Performance of \ours{} with different validation datasets for hyperparameter evaluation.
        All \ours{} runs above optimize hyperparameters for fine-tuning on CIFAR-10.
        \ours{} produces a robust fine-tuned model with all validation datasets, with the best results achieved when the validation set is from a different distribution than the fine-tuning dataset, CIFAR-10.
    }
\end{table}

==> sections/experiments_old.tex <==
\subsection{Experimental Setup}
\textbf{Datasets.} 
We evaluate \ours{} on a wide array of datasets with a distribution shift between training and test.
The datasets we consider include both synthetic and real-world distribution shifts.
Below, we summarize the datasets we use for evaluation, including the fine-tuning dataset (ID), the validation dataset for hyperparameter optimization, and the test OOD datasets.

\begin{itemize}
    \item \textbf{CIFAR-10} \citep{krizhevsky2009learning} contains 60,000 images across 10 classes.
    We use CIFAR-10 for fine-tuning, 100 examples from CIFAR-10-C for validation, and the CIFAR-10.1~\citep{recht2018cifar10.1,torralba2008tinyimages} and CIFAR-10.2~\citep{lu2020harder} as OOD test sets.

    \item \textbf{ImageNet} ~\citep{deng2009imagenet} contains over a million images in 1000 categories. 
    We use ImageNet as our ID distribution, 15000 examples from ImageNet-C for validation, and five ImageNet variations for the OOD datasets following prior works~\citep{clip,wortsman2022robust,kumar2022fine,goyal2022finetune}: ImageNet-V2~\citep{recht2019imagenet}, ImageNet-R~\citep{hendrycks2021many}, ImageNet-A~\citep{hendrycks2021natural}, ImageNet-Sketch~\citep{wang2019learning}, and ObjectNet \citep{barbu2019objectnet}.
    
    \item \textbf{WILDS-iWildCam} \citep{beery2021iwildcam, koh2021wilds, sagawa2022extending} is an animal image classification dataset with 182 classes. 
    Differences in camera specifications and attributes such as background and lighting distinguish ID and OOD.
    We use the ID train set from \citet{koh2021wilds} as the fine-tuning dataset, the OOD validation set for hyperparameter optimization, and the OOD test set for evaluation.

    \item \textbf{WILDS-FMoW} \citep{christie2018functional, koh2021wilds, sagawa2022extending} contains remote sensing imagery from satellites. 
    Each image is to be classified into one among 62 categories, including labels like ``impoverished settlement'' and ``hospital''.
    The ID and OOD datasets differ in time of acquisition and geographic location.
    We use the ID train set for fine-tuning, the OOD validation set for hyperparameter optimization, and the OOD test set for evaluation.

In all of the transfer learning datasets described below, we use a portion of the validation set for hyperparameter optimization.
    \item \textbf{Caltech101} \citep{fei2004learning} contains images of objects from 101 different categories, including ``dragonfly'', ``grand piano'', and ``saxophone.''

    \item \textbf{StanfordCars} \citep{krause20133d} features a collection of car images categorized by model, make, and year, where the task is to classify them into one of 196 types, such as ``Ford Mustang Convertible 1967'' or ``Toyota Prius Hatchback 2009.''

    \item \textbf{Flowers102} \citep{veeling2018rotation} consists of flower images from the UK, with the objective of classifying each image into one of 102 species, such as ``oxeye daisy'' or ``hibiscus.''

    \item \textbf{PatchCamelyon} \citep{veeling2018rotation} provides digital pathology images for binary classification, with the goal of identifying metastatic tumor tissues.

    \item \textbf{Rendered SST2} \citep{radford2021learning} is a dataset for optical character recognition, where the task is to classify text sentiment as ``positive'' or ``negative.''
    
\end{itemize}

\vspace{2mm} \noindent 
\textbf{Baselines.} 
We compare \ours{} against several methods for adapting pretrained models. 
We include two standard transfer learning methods that minimize cross-entropy loss: linear probing (LP) and full fine-tuning (FT).
We also compare with recent works in robust fine-tuning: L2-SP~\citep{li2018massively}, which fine-tunes with an L2 regularization term towards pretrained weights; LP-FT~\citep{kumar2022fine}, which performs linear probing followed by full fine-tuning; and FLYP~\citep{goyal2022finetune}, which fine-tunes with a contrastive loss.
We additionally evaluate all methods with weight ensembling~\citep{wortsman2022robust}, which is shown to improve OOD performance in an orthogonal way to other robust fine-tuning methods.

\vspace{2mm} \noindent 
\textbf{Models.} 
We fine-tune pre-trained CLIP~\citep{radford2021learning} models, including those provided in the \texttt{open-clip} repository~\citep{ilharco_gabriel_2021_5143773}. 
We use the CLIP ViT-B/16 model from OpenAI as our default model, unless specified otherwise. 
The CIFAR-10 experiments use the CLIP ViT-L/14 model from OpenAI.

\vspace{2mm} \noindent 
\textbf{Training.} 
We closely follow the training procedure described in~\citep{goyal2022finetune}.
All methods fine-tune models with an AdamW optimizer and a cosine learning rate scheduler. 
We use a batch size of 512 for ImageNet and 256 for all other datasets. 
For all baselines, we use learning rate and weight decays tuned through grid search and implement early stopping based on in-distribution (ID) validation accuracy. 
We note that all methods, including \ours{}, do not observe any of the test OOD datasets at training.
We report average metrics over 5 runs with 95\% confidence intervals. 
We use text templates used in prior work~\citep{radford2021learning,wortsman2022robust} to generate zero-shot final layer weights for all datasets.
A comprehensive breakdown of hyperparameter sweeps can be accessed in Appendix B.

\vspace{2mm} \noindent 
\textbf{\ours{}-specific settings.} 
% \ours{} uses a validation dataset different from both the reference (ID) dataset and the test OOD datasets for hyperparameter optimization.
As described in~\cref{sec:method}, \ours{} learns weights for nine different losses on a log-uniform range $[\text{1e-4},\text{1e2}]$, learning rate in the log-uniform range $[\text{1e-7},\text{1e-3}]$, and weight decay in the log-uniform range $[0.0, 1.0]$.
The layerwise variant of \ours{} learns per-layer learning rates and weight decay regularization terms, each sampled from the same respective range.
\todo{Add optuna hyperparames: inner loop steps, outer loop steps}

\subsection{Evaluation Under Distribution Shifts}

To evaluate the effectiveness of \ours{} in adapting pretrained models to new tasks, we compare against baselines on several large-scale, real-world distribution shift benchmarks, including ImageNet, WILDS-iWildCam, and WILDS-FMoW.
We report weight ensembling results with the mixture coefficient that attains the highest ID validation accuracy.
We report macro F1 score for WILDS-iWildCam and worst-region accuracy for WILDS-FMoW, following \citet{koh2021wilds}.

We report the ID and OOD test metrics of all methods in \cref{tab:big_distribution_shift_table}.
We find that \ours{} consistently outperforms all baselines on unseen OOD test distributions.
Additionally, these gains in OOD performance are preserved when ensembling the zeroshot and fine-tuned models, as proposed by \citet{wortsman2022robust}.

\textcolor{blue}{\ours{} attains a new state of the art on WILDS-iWildCam by $XXX\%$ in OOD Macro F1 score, using a ViT-L/14@336px backbone.}
With a ViT-B/16 model, \ours{} improves OOD performance by XXX\% over full fine-tuning (FT) and XXX\% over the current state-of-the-art, FLYP. 

Our experiments demonstrate that \ours{} consistently improves effective robustness on ImageNet, WILDS-iWildCam, and WILDS-FMoW compared to baseline methods.
\ours{} achieves superior out-of-distribution (OOD) accuracy compared to baseline methods for any given in-distribution (ID) accuracy on ImageNet.

\textbf{Weight ensembling curves.} We use the \textit{effective robustness} framework by \citet{taori2020measuring} to evaluate model robustness based on accuracy exceeding a baseline trained only on the reference distribution.

Linearly interpolating the weights of a fine-tuned model and a pretrained model (WiSE-FT) has been shown to improve both ID and OOD performance \citep{wortsman2022model}.
Hence, we include weight ensembling as an additional point of comparison, and interpolate the weights of models fine-tuned by each method with 10 mixing coefficients $\alpha$.
We use scatter plots to display effective robustness and plot the reference distribution accuracy (ID) against the shift accuracy (OOD) at various mixing coefficients.


\textbf{ImageNet distribution shifts.}

\textbf{WILDS distribution shifts.} 
We evaluate \ours{} on WILDS-iWildCam and CIFAR-10 distribution shifts in ~\cref{tab:iWildCam_no_ensembling_data_table} and ~\cref{tab:cifar10}, respectively.
\ours{} outperforms several representative methods for robust fine-tuning on unseen OOD data.

\input{tables/big_table.tex}

\textbf{CIFAR distribution shifts.}  We evaluate \ours{} on a CIFAR-10 derived distribution shift task and report results in ~\cref{tab:cifar10}.
We find that \ours{} outperforms several representative methods for robust fine-tuning on unseen synthetic OOD data.

\begin{table*}
\centering
\begin{tabular}{ccc}
\toprule
Method & CIFAR-10.1 & CIFAR-10.2 \\
\midrule
Zero-shot & 92.5 & 88.8 \\
Fine-tuning & 95.9 & 91.3 \\
\oursbf & \textbf{97.5} & \textbf{93.5} \\
\midrule
% WiSE-FT ($\alpha=0.5$) & 97.6 & 93.4 \\
WiSE-FT (best $\alpha$) & 98.0 & 94.4 \\
\oursbf w/ weight ensembling (best $\alpha$) & \textbf{98.3} & \textbf{95.0} \\
\bottomrule
\end{tabular}
\caption{CIFAR-10 results.}
\end{table*}


\begin{table*}[t] \centering
\begin{minipage}{.56\textwidth} \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{ccc}
    \toprule
    Method & CIFAR-10.1 & CIFAR-10.2 \\
    \midrule
    Zero-shot & 92.5 & 88.8 \\
    Fine-tuning & 95.9 & 91.3 \\
    \oursbf{} & \textbf{97.5} & \textbf{93.5} \\
    \midrule
    % WiSE-FT ($\alpha=0.5$) & 97.6 & 93.4 \\
    WiSE-FT (best $\alpha$) & 98.0 & 94.4 \\
    \oursbf{} w/ weight ensembling (best $\alpha$) & \textbf{98.3} & \textbf{95.0} \\
    \bottomrule
    \end{tabular}
    }
    \caption{
    \ours{} outperforms fine-tuning by $2.2\%$ on CIFAR-10.2 and by $1.4\%$ on CIFAR-10.1, using only 100 samples from CIFAR-10-C.
    \ours{} additionally outperforms WiSE-FT with weight ensembling.}
    \label{tab:cifar10}
\end{minipage}%
\hfill
\begin{minipage}{.42\textwidth} \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{cccc}
    \toprule
    Validation Dataset & CIFAR-10.1 & CIFAR-10.2 \\
    \midrule
    CIFAR-10-C & 97.4 (0.2) & 93.5 (0.2) \\
    CIFAR-10 & 96.9 (0.2) & 93.2 (0.1) \\
    CIFAR-10.1 & 96.8 (0.3) & 92.8 (0.2) \\
    CIFAR-10.2 & 96.7 (0.5) & 93.8 (0.0) \\
    \bottomrule
    \end{tabular}
    }
    \caption{
    ID and OOD performance of \ours{} using various validation sets for hyperparameter optimization.
    \ours{} uses just 100 samples from each of CIFAR-10-C, CIFAR-10, CIFAR-10.1, and CIFAR-10.2.}
    \label{tab:varying_validation_sets}
    \end{minipage}
\end{table*}


\subsection{Few-Shot Classification}

Few-shot classification is a critical benchmark for assessing the practicality of zeroshot models in many real-world applications, where limited labeled fine-tuning data is available.
\ours{} effectively generalizes given small quantities of labeled data, making it a promising approach for fine-tuning in low-data regimes.
\ours{} improves upon state-of-the-art fine-tuning methods in few-shot learning, resulting in gains of up to $5.1\%$ and $4.0\%$ on the SST2 and PatchCamelyon benchmarks, respectively.

\subsubsection{Binary Few-Shot Classification}

In few-shot binary classification, the small number of training examples present a challenging task for adaptation.
Our evaluation encompasses two datasets: PatchCamelyon and Rendered-SST2, replicating the experimental setup of \citet{radford2021learning}.
\ours{} significantly improves upon existing fine-tuning approaches in 4, 16, and 32 shot classification, as shown in \cref{tab:fewshot-binary-classification}. 
For example, \ours{} outperforms FLYP by $3.7\%$ and traditional full fine-tuning by $3.9\%$ in a difficult 4-shot classification task on SST2.

\input{tables/fewshot_binary.tex}

% \subsubsection{ImageNet Few-Shot Classification}

\subsection{Transfer Learning}


\input{tables/transfer_learning.tex}


Does \ours{} improve performance even when the test distribution is the same as the fine-tuning distribution?
We consider the more general transfer learning setup, where a model trained on one dataset is applied to a different, but related, dataset, with the aim of achieving high in-distribution accuracy.
\ours{} improves performance on XX out of XX transfer learning datasets, compared to several state-of-the-art fine-tuning methods.

In \cref{tab:transfer_learning}, we benchmark \ours{} against other models on six transfer learning datasets: PatchCamelyon, CalTech101, StanfordCars, Flowers102, ImageNet, and iWildCam. 
\ours{} shows superior generalization across all six datasets. For instance, \ours{} improves performance by $XX.XX\%$ than XXX baseline on XXX dataset and $XX.XX\%$ on XXX.


\subsection{Transferability of Hyperparameters} 

\subsection{Varying the Hyperparameter Optimization Dataset} 
We evaluate the performance of \ours{} using different validation datasets in \cref{tab:varying_validation_sets}.
While our main results optimize hyperparameters using a held-out validation set from a distribution that is different from the ID and test OOD distributions, here we use both a held-out ID validation set and a held-out OOD validation set.
We find that \ours{} exhibits strong test OOD performance with several different hyperparameter optimization datasets.
However, the best test OOD performance is attained with a validation set that is from a different distribution than the ID dataset.

% \begin{table}[]
% \centering
% \begin{tabular}{cccc}
% \toprule
% Validation Dataset & CIFAR-10.1 & CIFAR-10.2 \\
% \midrule
% CIFAR-10-C & 97.4 (0.2) & 93.5 (0.2) \\
% CIFAR-10 & 96.9 (0.2) & 93.2 (0.1) \\
% CIFAR-10.1 & 96.8 (0.3) & 92.8 (0.2) \\
% CIFAR-10.2 & 96.7 (0.5) & 93.8 (0.0) \\
% \bottomrule
% \end{tabular}
% \caption{
% ID and OOD performance of \ours{} using various validation sets for hyperparameter optimization.
% \ours{} uses just 100 samples from each of CIFAR-10-C, CIFAR-10, CIFAR-10.1, and CIFAR-10.2.}
% \label{tab:varying_validation_sets}
% \end{table}


% \subsection{Transferring Learned Hyperparameters Across Datasets}
% 1. Learned on CIFAR-10 -> CIFAR-10-C, finetune on CINIC, evaluate on CIFAR-10.1,10.2?

% 2. Learned on CIFAR-10 -> CIFAR-10-C, finetune on MNIST, evaluate on RMNIST,CMNIST,EMNIST,etc.?

% \input{tables/iWildCam}
% iWildCam state-of-the-art~\cref{tab:sota_iwild}

==> tables/big_table.tex <==
\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{@{}ccccccccc@{}}
\toprule
& \multicolumn{4}{c}{iWILDCam} & \multicolumn{4}{c}{FMoW} \\ \cmidrule(l){2-9} 
& \multicolumn{2}{c}{Without Ensembling} & \multicolumn{2}{c|}{With Ensembling} & \multicolumn{2}{c}{Without Ensembling} & \multicolumn{2}{c}{With Ensembling} \\ 
\cmidrule(lr){2-3}  \cmidrule(lr){4-5}  \cmidrule(lr){6-7}  \cmidrule(lr){8-9} 
\multirow{-3}{*}{Methods} & ID & OOD & ID & \multicolumn{1}{c|}{OOD} & ID & OOD & ID & OOD \\ \midrule
Zeroshot & 8.7 (-) & 11.0 (-) & 8.7 (-) & \multicolumn{1}{c|}{11.0 (-)} & 20.4 (-) & 18.7 (-) & 20.4 (-) & 18.7 (-) \\
LP & 44.5 (0.6) & 31.1 (0.4) & 45.5 (0.6) & \multicolumn{1}{c|}{31.7 (0.4)} & 48.2 (0.1) & 30.5 (0.3) & 48.5 (0.1) & 30.7 (0.3) \\
FT & 48.1 (0.5) & 35.0 (0.5) & 48.1 (0.5) & \multicolumn{1}{c|}{35.0 (0.5)} & 68.5 (0.1) & 39.2 (0.7) & 68.5 (0.1) & 39.2 (0.7)\\
L2-SP & 48.6 (0.4) & 35.3 (0.3) & 48.6 (0.4) & \multicolumn{1}{c|}{35.3 (0.3)} & 68.6 (0.1) & 39.4 (0.6) & 68.6 (0.1) & 39.4 (0.6) \\
LP-FT & 49.7 (0.5) & 34.7 (0.4) & 50.2 (0.5) & \multicolumn{1}{c|}{35.7 (0.4)} & 68.4 (0.2) & 40.4 (1.0) & 68.4 (0.2) & 40.4 (1.0) \\
FLYP & \textbf{52.2 (0.6)} & 35.6 (1.2) & \textbf{52.5 (0.6)} & \multicolumn{1}{c|}{37.1 (1.2)} & \textbf{68.6 (0.2)} & 41.3 (0.8) & \textbf{69.0 (0.1)} & 41.9 (0.7) \\ \midrule
\oursbf{} & 51.0 (0.5) & \textbf{38.3 (0.5)} & 51.3 (0.5)  & \textbf{39.3 (0.5)} & 67.1 (0.3) & \textbf{42.3 (0.5)} & 67.1 (0.3) & \textbf{42.3 (0.5)} \\
\bottomrule
\end{tabular}
}
\caption{
\ours{} outperforms all baselines both with and without ensembling.
Without ensembling, \ours{} improves OOD performance by $3.7\%$ on WILDS-iWildCam and $6.1\%$ on WILDS-FMoW, respectively. 
On WILDS-iWildCam, these improvements are preserved with ensembling, leading to an increase of $2.2\%$ in OOD macro F1.
}
\label{tab:big_distribution_shift_table}

==> tables/fewshot_binary.tex <==
\begin{table*}[t!]
\centering
% \resizebox{1.03\linewidth}{!}{
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{3}{c}{PatchCamelyon} & \multicolumn{3}{c}{SST2} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
$k$ (shots) & 4 & 16 & 32 & 4 & 16 & 32 \\
\midrule
Zeroshot & 56.5 (-) & 56.5 (-) & 56.5 (-) & 60.5 (-) & 60.5 (-) & 60.5 (-) \\
LP & 60.4 (4.0) & 64.4 (3.7) & 67.0 (4.4) & 60.8 (1.8) & 61.9 (1.4) & 62.9 (1.3) \\
FT & 63.1 (5.5) & 71.6 (4.6) & 75.2 (3.7) & 61.1 (0.7) & 62.4 (1.6) & 63.4 (1.9) \\
LP-FT & 62.7 (5.3) & 69.8 (5.3) & 73.9 (4.6) & 60.9 (2.4) & 62.9 (1.9) & 63.6 (1.4) \\
FLYP & 66.9 (5.0) & 74.5 (2.0) & 76.4 (2.4) & 61.3 (2.7) & 65.6 (2.1) & 68.0 (1.7) \\
\midrule
% \rowcolor[gray]{0.8}
\oursbf{} & \textbf{68.1 (5.1)} & \textbf{76.8 (2.9)} & \textbf{79.5 (2.0)} & \textbf{65.0 (3.8)} & \textbf{67.5 (1.1)} & \textbf{69.0 (1.1)} \\
\bottomrule
\end{tabular}
% }
\vspace{-2mm}
\caption{In binary few-shot classification, \ours{} outperforms existing robust fine-tuning methods. 
\ours{} outperforms FLYP by $3.1\%$ and full fine-tuning by $4.3\%$ in 32-shot classification on PatchCamelyon.
}
\label{tab:fewshot-binary-classification}
\end{table*}
